Periodicity shadows II. Computational aspects

This article provides the second part of the research initiated in arXiv:2411.17381, where we introduced and investigated so called periodicity shadows, which are special skew-symmetric matrices related to symmetric algebras with periodic simple modules. In arXiv:2411.17381 we focused on theoretical aspects, whereas here we present complementary cosiderations concerning computational issues. Namely, we discuss an algorithm, which computes all tame periodicity shadows of given size (see Section 2), and then present lists of all tame periodicity shadows of small sizes, that is at most 6.

==> m3_ps45_short.tex <==
\resizebox{.5\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  1 \\
     2 &  0 & -1 \\
    -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\  2  v  \end{bmatrix}
  \begin{bmatrix}
    c & c &  2  c  \\
    \cdot & c &  2  c  \\
    \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\resizebox{.5\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 &  1 \\
     1 &  0 & -1 \\
    -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
    c & c & c \\
    \cdot & c & c \\
    \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\resizebox{.5\linewidth}{!}{%
$
  \begin{bmatrix}
     0 &  0 &  0 \\
     0 &  0 &  0 \\
     0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\ v_{3} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{2} & c_{3} \\
    \cdot & c_{4} & c_{5} \\
    \cdot & \cdot & c_{6} \\
  \end{bmatrix}
$
}


==> m3_ps_not45_short.tex <==
\resizebox{.5\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  2 \\
     2 &  0 & -2 \\
    -2 &  2 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
    c & c & c \\
    \cdot & c & c \\
    \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\resizebox{.5\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  1 \\
     2 &  0 & -2 \\
    -1 &  2 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v  \\ v \\  2  v  \end{bmatrix}
  \begin{bmatrix}
     4  c  &  2  c  &  4  c  \\
    \cdot & c &  2  c  \\
    \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}


==> m4_ps45_long.tex <==
\resizebox{\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  1 &  1 \\
     2 &  0 & -1 & -1 \\
    -1 &  1 &  0 &  0 \\
    -1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{1} \\  - v_{2}   +  2  v_{1}   \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{1} &  - c_{2}   +  2  c_{1}   & c_{2} \\
    \cdot & c_{1} &  - c_{2}   +  2  c_{1}   & c_{2} \\
    \cdot & \cdot & c_{3}  -4  c_{2}   +  4  c_{1}   &  - c_{3}   +  2  c_{2}   \\
    \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\resizebox{\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 \\
     1 &  1 &  0 & -1 \\
    -1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2}  - v_{1}   \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{2}  - c_{1}   & c_{1} & c_{2} \\
    \cdot & c_{3}  -2  c_{2}   + c_{1}  & c_{2}  - c_{1}   & c_{3}  - c_{2}   \\
    \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\resizebox{\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  1 \\
     1 &  0 &  0 & -1 \\
     1 &  0 &  0 & -1 \\
    -1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2}  - v_{1}   \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3}  - c_{2}   & c_{2} & c_{3} \\
    \cdot & c_{3}  -2  c_{2}   + c_{1}  & c_{2}  - c_{1}   & c_{3}  - c_{2}   \\
    \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}



==> m4_ps45_short.tex <==
\resizebox{.5\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 \\
     2 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 \\
    -1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{1} \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\resizebox{.5\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 \\
     0 &  1 &  0 & -1 \\
    -1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{2} & c_{1} & c_{2} \\
    \cdot & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\resizebox{.5\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 &  0 &  1 \\
     1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 \\
    -1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} & c_{2} & c_{3} \\
    \cdot & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\resizebox{.5\linewidth}{!}{%
$
  \begin{bmatrix}
     0 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\ v_{3} \\ v_{4} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{2} & c_{3} & c_{4} \\
    \cdot & c_{5} & c_{6} & c_{7} \\
    \cdot & \cdot & c_{8} & c_{9} \\
    \cdot & \cdot & \cdot & c_{10} \\
  \end{bmatrix}
$
}


==> m4_ps_not45_long.tex <==
\resizebox{\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  2 \\
     2 &  0 & -1 & -1 \\
     0 &  1 &  0 & -1 \\
    -2 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\  - v_{2}   +  2  v_{1}   \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{2} &  - c_{2}   +  2  c_{1}   & c_{2} \\
    \cdot & c_{3} &  - c_{3}   +  2  c_{2}   & c_{3} \\
    \cdot & \cdot & c_{3}  -4  c_{2}   +  4  c_{1}   &  - c_{3}   +  2  c_{2}   \\
    \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}



==> m4_ps_not45_short.tex <==
\resizebox{.5\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 \\
     2 &  0 & -2 &  0 \\
     0 &  2 &  0 & -1 \\
    -1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{1} \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{2} & c_{3} &  2  c_{2}  \\
    \cdot & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\resizebox{.5\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 \\
     2 &  0 &  0 & -2 \\
     0 &  0 &  0 &  0 \\
    -1 &  2 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{1}  \\ v_{1} \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     4  c_{1}  &  2  c_{1}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\resizebox{.5\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  2 \\
     2 &  0 & -2 &  0 \\
     0 &  2 &  0 & -2 \\
    -2 &  0 &  2 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{2} & c_{1} & c_{2} \\
    \cdot & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\resizebox{.5\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  2 \\
     2 &  0 &  0 & -2 \\
     0 &  0 &  0 &  0 \\
    -2 &  2 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} & c_{2} & c_{3} \\
    \cdot & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}


==> m5_notps_short.tex <==
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -2 &  0 &  0 \\
     0 &  2 &  0 & -1 & -1 \\
     0 &  0 &  1 &  0 & -1 \\
    -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v  \\ v \\  2  v  \\  0  \\  2  v  \end{bmatrix}
  \begin{bmatrix}
     4  c  &  2  c  &  4  c  &  0  &  4  c  \\
    \cdot & c &  2  c  &  0  &  2  c  \\
    \cdot & \cdot &  4  c  &  0  &  4  c  \\
    \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -2 &  0 &  0 \\
     0 &  2 &  0 &  0 & -2 \\
     0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  2 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  0  \\ v \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c &  0  \\
    \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 & -1 \\
     0 &  1 &  0 & -1 & -1 \\
     0 &  1 &  1 &  0 & -1 \\
    -1 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v  \\  - v  \\  - v  \\ v \\  -2  v  \end{bmatrix}
  \begin{bmatrix}
    c & c & c &  - c  &  2  c  \\
    \cdot & c & c &  - c  &  2  c  \\
    \cdot & \cdot & c &  - c  &  2  c  \\
    \cdot & \cdot & \cdot & c &  -2  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 & -1 \\
     0 &  1 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 & -1 \\
    -1 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  - v  \\ v \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c &  - c  &  0  \\
    \cdot & \cdot & \cdot & c &  0  \\
    \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 &  0 \\
     0 &  1 &  0 & -1 & -1 \\
     0 &  1 &  1 &  0 & -1 \\
    -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  - v  \\  - v  \\ v \\  -2  v  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot & c & c &  - c  &  2  c  \\
    \cdot & \cdot & c &  - c  &  2  c  \\
    \cdot & \cdot & \cdot & c &  -2  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 &  0 \\
     0 &  1 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 & -1 \\
    -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  - v  \\ v \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c &  - c  &  0  \\
    \cdot & \cdot & \cdot & c &  0  \\
    \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 & -1 \\
     0 &  1 &  0 & -1 & -1 \\
     0 &  0 &  1 &  0 & -1 \\
    -1 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  -2  v  \\  - v  \\  -2  v  \\ v \\  -2  v  \end{bmatrix}
  \begin{bmatrix}
     4  c  &  2  c  &  4  c  &  -2  c  &  4  c  \\
    \cdot & c &  2  c  &  - c  &  2  c  \\
    \cdot & \cdot &  4  c  &  -2  c  &  4  c  \\
    \cdot & \cdot & \cdot & c &  -2  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 & -1 \\
     0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  0  \\ v \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c &  0  \\
    \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 \\
     0 &  1 &  0 & -1 & -1 \\
     0 &  0 &  1 &  0 & -1 \\
    -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v  \\  - v  \\  -2  v  \\ v \\  -2  v  \end{bmatrix}
  \begin{bmatrix}
    c & c &  2  c  &  - c  &  2  c  \\
    \cdot & c &  2  c  &  - c  &  2  c  \\
    \cdot & \cdot &  4  c  &  -2  c  &  4  c  \\
    \cdot & \cdot & \cdot & c &  -2  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 \\
     0 &  1 &  0 &  0 & -2 \\
     0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  2 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  0  \\ v \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c &  0  \\
    \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 \\
     0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  0  \\ v \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c &  0  \\
    \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  2 \\
     2 &  0 & -1 & -1 & -1 \\
     0 &  1 &  0 & -1 & -1 \\
     0 &  1 &  1 &  0 & -1 \\
    -2 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\  2  v  \\  0  \\  0  \\  2  v  \end{bmatrix}
  \begin{bmatrix}
    c &  2  c  &  0  &  0  &  2  c  \\
    \cdot &  4  c  &  0  &  0  &  4  c  \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  2 \\
     2 &  0 & -1 & -1 & -1 \\
     0 &  1 &  0 & -1 &  0 \\
     0 &  1 &  1 &  0 & -1 \\
    -2 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\  0  \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
    c & c &  0  & c & c \\
    \cdot & c &  0  & c & c \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  2 \\
     2 &  0 & -1 & -1 &  0 \\
     0 &  1 &  0 & -1 & -1 \\
     0 &  1 &  1 &  0 & -1 \\
    -2 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v \\  0  \\  0  \\ v \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot & c &  0  &  0  & c \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 & -1 \\
     0 &  1 &  0 & -1 & -1 \\
    -1 &  1 &  1 &  0 & -1 \\
    -1 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\  0  \\  2  v  \\  - v  \\ v \end{bmatrix}
  \begin{bmatrix}
    c &  0  &  2  c  &  - c  & c \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  4  c  &  -2  c  &  2  c  \\
    \cdot & \cdot & \cdot & c &  - c  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 & -1 \\
     0 &  1 &  0 & -1 & -1 \\
    -1 &  1 &  1 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  0  \\  - v  \\ v \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c &  - c  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 & -1 \\
     0 &  1 &  0 & -1 &  0 \\
    -1 &  1 &  1 &  0 &  0 \\
    -1 &  1 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\  0  \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
    c & c &  0  & c & c \\
    \cdot & c &  0  & c & c \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 & -1 \\
     0 &  1 &  0 & -1 &  0 \\
    -1 &  1 &  1 &  0 &  1 \\
    -1 &  1 &  0 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v \\  -2  v  \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot & c &  -2  c  & c & c \\
    \cdot & \cdot &  4  c  &  -2  c  &  -2  c  \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 & -1 \\
     0 &  1 &  0 & -1 &  1 \\
    -1 &  1 &  1 &  0 &  0 \\
    -1 &  1 & -1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v  \\  2  v  \\  0  \\  3  v  \\ v \end{bmatrix}
  \begin{bmatrix}
     4  c  &  4  c  &  0  &  6  c  &  2  c  \\
    \cdot &  4  c  &  0  &  6  c  &  2  c  \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot &  9  c  &  3  c  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 & -1 \\
     0 &  1 &  0 & -1 &  1 \\
    -1 &  1 &  1 &  0 &  1 \\
    -1 &  1 & -1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\  2  v  \\  -2  v  \\  3  v  \\ v \end{bmatrix}
  \begin{bmatrix}
    c &  2  c  &  -2  c  &  3  c  & c \\
    \cdot &  4  c  &  -4  c  &  6  c  &  2  c  \\
    \cdot & \cdot &  4  c  &  -6  c  &  -2  c  \\
    \cdot & \cdot & \cdot &  9  c  &  3  c  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 &  0 \\
     0 &  1 &  0 & -1 & -1 \\
    -1 &  1 &  1 &  0 & -1 \\
    -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\ v \\  - v  \\ v \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c &  - c  & c \\
    \cdot & \cdot & \cdot & c &  - c  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 &  0 \\
     0 &  1 &  0 & -1 & -1 \\
    -1 &  1 &  1 &  0 &  0 \\
    -1 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v  \\  0  \\  - v  \\  - v  \\ v \end{bmatrix}
  \begin{bmatrix}
    c &  0  & c & c &  - c  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c & c &  - c  \\
    \cdot & \cdot & \cdot & c &  - c  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 &  0 \\
     0 &  1 &  0 & -1 & -1 \\
    -1 &  1 &  1 &  0 &  1 \\
    -1 &  0 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  -2  v  \\  0  \\  -3  v  \\  - v  \\ v \end{bmatrix}
  \begin{bmatrix}
     4  c  &  0  &  6  c  &  2  c  &  -2  c  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  9  c  &  3  c  &  -3  c  \\
    \cdot & \cdot & \cdot & c &  - c  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 \\
     2 &  0 &  0 & -1 & -1 \\
     0 &  0 &  0 & -1 &  1 \\
    -1 &  1 &  1 &  0 &  0 \\
    -1 &  1 & -1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\  0  \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
    c & c &  0  & c & c \\
    \cdot & c &  0  & c & c \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 \\
     2 &  0 &  0 & -1 & -1 \\
     0 &  0 &  0 & -1 &  1 \\
    -1 &  1 &  1 &  0 &  1 \\
    -1 &  1 & -1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\  - v  \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
    c & c &  - c  & c & c \\
    \cdot & c &  - c  & c & c \\
    \cdot & \cdot & c &  - c  &  - c  \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 \\
     2 &  0 &  0 & -1 & -1 \\
     0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  0 &  0 & -1 \\
    -1 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\ v \\  0  \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c &  0  &  0  \\
    \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  1 &  1 &  1 \\
     2 &  0 & -1 & -1 & -1 \\
    -1 &  1 &  0 & -1 & -1 \\
    -1 &  1 &  1 &  0 & -1 \\
    -1 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\  2  v  \\  -2  v  \\  2  v  \end{bmatrix}
  \begin{bmatrix}
    c & c &  2  c  &  -2  c  &  2  c  \\
    \cdot & c &  2  c  &  -2  c  &  2  c  \\
    \cdot & \cdot &  4  c  &  -4  c  &  4  c  \\
    \cdot & \cdot & \cdot &  4  c  &  -4  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  1 &  1 &  1 \\
     2 &  0 & -1 & -1 & -1 \\
    -1 &  1 &  0 & -1 & -1 \\
    -1 &  1 &  1 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  0  \\  - v  \\ v \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c &  - c  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  1 &  1 &  1 \\
     2 &  0 & -1 & -1 & -1 \\
    -1 &  1 &  0 & -1 &  0 \\
    -1 &  1 &  1 &  0 & -1 \\
    -1 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\ v \\  0  \\ v \end{bmatrix}
  \begin{bmatrix}
    c & c & c &  0  & c \\
    \cdot & c & c &  0  & c \\
    \cdot & \cdot & c &  0  & c \\
    \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  1 &  1 &  1 \\
     2 &  0 & -1 & -1 & -1 \\
    -1 &  1 &  0 & -1 &  0 \\
    -1 &  1 &  1 &  0 &  0 \\
    -1 &  1 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\  0  \\  0  \\  2  v  \end{bmatrix}
  \begin{bmatrix}
    c & c &  0  &  0  &  2  c  \\
    \cdot & c &  0  &  0  &  2  c  \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 & -1 \\
     1 &  1 &  0 & -1 & -1 \\
     1 &  1 &  1 &  0 & -1 \\
    -1 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\  - v  \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
    c & c &  - c  & c & c \\
    \cdot & c &  - c  & c & c \\
    \cdot & \cdot & c &  - c  &  - c  \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 & -1 \\
     1 &  1 &  0 & -1 &  0 \\
     1 &  1 &  1 &  0 & -1 \\
    -1 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v  \\  0  \\  - v  \\  2  v  \\ v \end{bmatrix}
  \begin{bmatrix}
     4  c  &  0  &  -2  c  &  4  c  &  2  c  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c &  -2  c  &  - c  \\
    \cdot & \cdot & \cdot &  4  c  &  2  c  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 & -1 \\
     1 &  1 &  0 & -1 &  1 \\
     1 &  1 &  1 &  0 & -1 \\
    -1 &  1 & -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  3  v  \\  - v  \\  - v  \\  3  v  \\ v \end{bmatrix}
  \begin{bmatrix}
     9  c  &  -3  c  &  -3  c  &  9  c  &  3  c  \\
    \cdot & c & c &  -3  c  &  - c  \\
    \cdot & \cdot & c &  -3  c  &  - c  \\
    \cdot & \cdot & \cdot &  9  c  &  3  c  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 & -1 \\
     1 &  1 &  0 &  0 & -1 \\
     1 &  1 &  0 &  0 & -1 \\
    -1 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  - v  \\ v \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c &  - c  &  0  \\
    \cdot & \cdot & \cdot & c &  0  \\
    \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 &  0 \\
     1 &  1 &  0 & -1 & -1 \\
     1 &  1 &  1 &  0 & -1 \\
    -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v \\  0  \\  0  \\ v \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot & c &  0  &  0  & c \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 &  0 \\
     1 &  1 &  0 & -1 &  0 \\
     1 &  1 &  1 &  0 & -1 \\
    -1 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\  0  \\  0  \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
    c &  0  &  0  & c & c \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 &  1 \\
     1 &  1 &  0 & -1 & -1 \\
     1 &  1 &  1 &  0 & -1 \\
    -1 & -1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v  \\ v \\ v \\  - v  \\ v \end{bmatrix}
  \begin{bmatrix}
    c &  - c  &  - c  & c &  - c  \\
    \cdot & c & c &  - c  & c \\
    \cdot & \cdot & c &  - c  & c \\
    \cdot & \cdot & \cdot & c &  - c  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 &  1 \\
     1 &  1 &  0 &  0 & -1 \\
     1 &  1 &  0 &  0 & -1 \\
    -1 & -1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  - v  \\ v \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c &  - c  &  0  \\
    \cdot & \cdot & \cdot & c &  0  \\
    \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 & -1 \\
     1 &  1 &  0 & -1 & -1 \\
     1 &  0 &  1 &  0 & -1 \\
    -1 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v  \\ v \\  0  \\ v \\  2  v  \end{bmatrix}
  \begin{bmatrix}
     4  c  &  2  c  &  0  &  2  c  &  4  c  \\
    \cdot & c &  0  & c &  2  c  \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c &  2  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 & -1 \\
     1 &  1 &  0 & -1 &  0 \\
     1 &  0 &  1 &  0 & -1 \\
    -1 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\  0  \\  0  \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
    c &  0  &  0  & c & c \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 & -1 \\
     1 &  1 &  0 & -1 &  1 \\
     1 &  0 &  1 &  0 & -1 \\
    -1 &  1 & -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ \frac{ -1 }{ 2 } v  \\  0  \\ \frac{ 3 }{ 2 } v  \\ v \end{bmatrix}
  \begin{bmatrix}
     -2  c  & c &  0  &  -3  c  &  -2  c  \\
    \cdot & \frac{ -1 }{ 2 } c  &  0  & \frac{ 3 }{ 2 } c  & c \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \frac{ -9 }{ 2 } c  &  -3  c  \\
    \cdot & \cdot & \cdot & \cdot &  -2  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 & -1 \\
     1 &  1 &  0 &  0 & -1 \\
     1 &  0 &  0 &  0 & -1 \\
    -1 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\  0  \\  0  \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
    c &  0  &  0  & c & c \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 & -1 \\
     1 &  1 &  0 &  1 & -1 \\
     1 &  0 & -1 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v  \\  0  \\  - v  \\ v \\  0  \end{bmatrix}
  \begin{bmatrix}
    c &  0  & c &  - c  &  0  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c &  - c  &  0  \\
    \cdot & \cdot & \cdot & c &  0  \\
    \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 & -1 \\
     1 &  1 &  0 &  1 & -1 \\
     1 &  0 & -1 &  0 &  1 \\
    -1 &  1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  -2  v  \\ v \\  -2  v  \\ v \\  0  \end{bmatrix}
  \begin{bmatrix}
     4  c  &  -2  c  &  4  c  &  -2  c  &  0  \\
    \cdot & c &  -2  c  & c &  0  \\
    \cdot & \cdot &  4  c  &  -2  c  &  0  \\
    \cdot & \cdot & \cdot & c &  0  \\
    \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 &  0 \\
     1 &  1 &  0 & -1 & -1 \\
     1 &  0 &  1 &  0 & -1 \\
    -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\ v \\  0  \\  2  v  \end{bmatrix}
  \begin{bmatrix}
    c & c & c &  0  &  2  c  \\
    \cdot & c & c &  0  &  2  c  \\
    \cdot & \cdot & c &  0  &  2  c  \\
    \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 &  0 \\
     1 &  1 &  0 & -1 &  0 \\
     1 &  0 &  1 &  0 & -1 \\
    -1 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\  0  \\ v \\ v \\  2  v  \end{bmatrix}
  \begin{bmatrix}
    c &  0  & c & c &  2  c  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c & c &  2  c  \\
    \cdot & \cdot & \cdot & c &  2  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 &  0 \\
     1 &  1 &  0 & -1 &  1 \\
     1 &  0 &  1 &  0 & -1 \\
    -1 &  0 & -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\  - v  \\ v \\  2  v  \\  2  v  \end{bmatrix}
  \begin{bmatrix}
    c &  - c  & c &  2  c  &  2  c  \\
    \cdot & c &  - c  &  -2  c  &  -2  c  \\
    \cdot & \cdot & c &  2  c  &  2  c  \\
    \cdot & \cdot & \cdot &  4  c  &  4  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 &  0 \\
     1 &  1 &  0 &  0 & -1 \\
     1 &  0 &  0 &  0 & -1 \\
    -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\  0  \\ v \\  0  \\ v \end{bmatrix}
  \begin{bmatrix}
    c &  0  & c &  0  & c \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c &  0  & c \\
    \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 &  1 \\
     1 &  1 &  0 & -1 & -1 \\
     1 &  0 &  1 &  0 & -1 \\
    -1 & -1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  - v  \\  -2  v  \\ v \\  -2  v  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot & c &  2  c  &  - c  &  2  c  \\
    \cdot & \cdot &  4  c  &  -2  c  &  4  c  \\
    \cdot & \cdot & \cdot & c &  -2  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 &  1 \\
     1 &  1 &  0 & -1 &  0 \\
     1 &  0 &  1 &  0 & -1 \\
    -1 & -1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\ v \\  0  \\ v \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c &  0  & c \\
    \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 &  1 \\
     1 &  1 &  0 &  0 & -1 \\
     1 &  0 &  0 &  0 & -1 \\
    -1 & -1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\  0  \\  2  v  \\  - v  \\ v \end{bmatrix}
  \begin{bmatrix}
    c &  0  &  2  c  &  - c  & c \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  4  c  &  -2  c  &  2  c  \\
    \cdot & \cdot & \cdot & c &  - c  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  1 & -1 \\
     1 &  1 &  0 & -1 & -1 \\
     1 & -1 &  1 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\  0  \\ \frac{ 1 }{ 2 } v  \\ \frac{ 3 }{ 2 } v  \end{bmatrix}
  \begin{bmatrix}
     4  c  &  4  c  &  0  &  2  c  &  6  c  \\
    \cdot &  4  c  &  0  &  2  c  &  6  c  \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c &  3  c  \\
    \cdot & \cdot & \cdot & \cdot &  9  c  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  1 & -1 \\
     1 &  1 &  0 & -1 & -1 \\
     1 & -1 &  1 &  0 &  1 \\
    -1 &  1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\  3  v  \\  - v  \\ v \\  3  v  \end{bmatrix}
  \begin{bmatrix}
    c &  3  c  &  - c  & c &  3  c  \\
    \cdot &  9  c  &  -3  c  &  3  c  &  9  c  \\
    \cdot & \cdot & c &  - c  &  -3  c  \\
    \cdot & \cdot & \cdot & c &  3  c  \\
    \cdot & \cdot & \cdot & \cdot &  9  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  1 & -1 \\
     1 &  1 &  0 & -1 &  0 \\
     1 & -1 &  1 &  0 &  0 \\
    -1 &  1 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\  0  \\  2  v  \\  3  v  \end{bmatrix}
  \begin{bmatrix}
    c & c &  0  &  2  c  &  3  c  \\
    \cdot & c &  0  &  2  c  &  3  c  \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot &  4  c  &  6  c  \\
    \cdot & \cdot & \cdot & \cdot &  9  c  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  1 & -1 \\
     1 &  1 &  0 & -1 &  1 \\
     1 & -1 &  1 &  0 &  0 \\
    -1 &  1 & -1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  0  \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  0 \\
     1 &  1 &  0 & -1 &  0 \\
     0 &  1 &  1 &  0 & -1 \\
    -1 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\  0  \\  0  \\ v \\  0  \end{bmatrix}
  \begin{bmatrix}
    c &  0  &  0  & c &  0  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c &  0  \\
    \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  0 \\
     1 &  1 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 & -1 \\
    -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v \\  0  \\  0  \\ v \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot & c &  0  &  0  & c \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  1 \\
     1 &  1 &  0 & -1 & -1 \\
     0 &  1 &  1 &  0 & -1 \\
    -1 & -1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\  0  \\  0  \\ v \\  0  \end{bmatrix}
  \begin{bmatrix}
    c &  0  &  0  & c &  0  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c &  0  \\
    \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  1 \\
     1 &  1 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 & -1 \\
    -1 & -1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v \\  0  \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot & c &  0  & c & c \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 & -1 \\
     1 &  1 &  0 & -1 &  0 \\
     0 &  0 &  1 &  0 & -1 \\
    -1 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v  \\  0  \\ v \\  2  v  \\ v \end{bmatrix}
  \begin{bmatrix}
     4  c  &  0  &  2  c  &  4  c  &  2  c  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c &  2  c  & c \\
    \cdot & \cdot & \cdot &  4  c  &  2  c  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 & -1 \\
     1 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  0  \\ v \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c &  0  \\
    \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 \\
     1 &  1 &  0 & -1 & -1 \\
     0 &  0 &  1 &  0 & -1 \\
    -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\  0  \\ v \\  0  \\ v \end{bmatrix}
  \begin{bmatrix}
    c &  0  & c &  0  & c \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c &  0  & c \\
    \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 \\
     1 &  1 &  0 & -1 &  0 \\
     0 &  0 &  1 &  0 & -1 \\
    -1 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\  0  \\ v \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
    c &  0  & c & c & c \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c & c & c \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  1 \\
     1 &  1 &  0 & -1 & -1 \\
     0 &  0 &  1 &  0 & -1 \\
    -1 & -1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\ v \\  - v  \\ v \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c &  - c  & c \\
    \cdot & \cdot & \cdot & c &  - c  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  1 & -1 \\
     1 &  1 &  0 & -1 & -1 \\
     0 & -1 &  1 &  0 &  1 \\
    -1 &  1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\  2  v  \\  0  \\ v \\  2  v  \end{bmatrix}
  \begin{bmatrix}
    c &  2  c  &  0  & c &  2  c  \\
    \cdot &  4  c  &  0  &  2  c  &  4  c  \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c &  2  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  1 & -1 \\
     1 &  1 &  0 & -1 &  0 \\
     0 & -1 &  1 &  0 & -1 \\
    -1 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\  0  \\ v \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
    c &  0  & c & c & c \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c & c & c \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  1 & -1 \\
     1 &  1 &  0 & -1 &  0 \\
     0 & -1 &  1 &  0 &  1 \\
    -1 &  1 &  0 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v \\  0  \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot & c &  0  & c & c \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  1 &  0 \\
     1 &  1 &  0 & -1 & -1 \\
     0 & -1 &  1 &  0 & -1 \\
    -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\  0  \\ v \\  0  \\ v \end{bmatrix}
  \begin{bmatrix}
    c &  0  & c &  0  & c \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c &  0  & c \\
    \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  1 &  0 \\
     1 &  1 &  0 & -1 & -1 \\
     0 & -1 &  1 &  0 &  0 \\
    -1 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\ v \\  0  \\  2  v  \end{bmatrix}
  \begin{bmatrix}
    c & c & c &  0  &  2  c  \\
    \cdot & c & c &  0  &  2  c  \\
    \cdot & \cdot & c &  0  &  2  c  \\
    \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  1 &  0 \\
     1 &  1 &  0 & -1 & -1 \\
     0 & -1 &  1 &  0 &  1 \\
    -1 &  0 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v \\  0  \\  0  \\ v \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  \\
    \cdot & c &  0  &  0  & c \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  1 \\
     1 &  0 &  0 & -1 & -1 \\
     1 &  0 &  0 &  1 & -1 \\
     0 &  1 & -1 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v  \\ v \\ v \\  0  \\  2  v  \end{bmatrix}
  \begin{bmatrix}
     4  c  &  2  c  &  2  c  &  0  &  4  c  \\
    \cdot & c & c &  0  &  2  c  \\
    \cdot & \cdot & c &  0  &  2  c  \\
    \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  1 \\
     1 &  0 &  0 & -1 &  0 \\
     1 &  0 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 & -1 \\
    -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\  0  \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
    c & c &  0  & c & c \\
    \cdot & c &  0  & c & c \\
    \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  1 \\
     1 &  0 &  0 &  0 & -1 \\
     1 &  0 &  0 &  1 & -1 \\
     0 &  0 & -1 &  0 &  1 \\
    -1 &  1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\  0  \\ v \\  0  \\ v \end{bmatrix}
  \begin{bmatrix}
    c &  0  & c &  0  & c \\
    \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c &  0  & c \\
    \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%


==> m5_ps_not45_long.tex <==
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.94\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  2 \\
     2 &  0 & -1 & -1 & -1 \\
     0 &  1 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 & -1 \\
    -2 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{3} \\  - v_{2}   - v_{3}   +  2  v_{1}   \\ v_{2} \\ v_{3} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{3} &  - c_{2}   - c_{3}   +  2  c_{1}   & c_{2} & c_{3} \\
    \cdot & c_{6} &  - c_{5}   - c_{6}   +  2  c_{3}   & c_{5} & c_{6} \\
    \cdot & \cdot & c_{4}  +  2  c_{5}   -4  c_{2}   + c_{6}  -4  c_{3}   +  4  c_{1}   &  - c_{4}   - c_{5}   +  2  c_{2}   &  - c_{5}   - c_{6}   +  2  c_{3}   \\
    \cdot & \cdot & \cdot & c_{4} & c_{5} \\
    \cdot & \cdot & \cdot & \cdot & c_{6} \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.94\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  2 \\
     2 &  0 & -1 & -1 &  0 \\
     0 &  1 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 & -1 \\
    -2 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{3} \\  - v_{2}   +  2  v_{1}   \\ v_{2} \\ v_{3} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{3} &  - c_{2}   +  2  c_{1}   & c_{2} & c_{3} \\
    \cdot & c_{6} &  - c_{5}   +  2  c_{3}   & c_{5} & c_{6} \\
    \cdot & \cdot & c_{4}  -4  c_{2}   +  4  c_{1}   &  - c_{4}   +  2  c_{2}   &  - c_{5}   +  2  c_{3}   \\
    \cdot & \cdot & \cdot & c_{4} & c_{5} \\
    \cdot & \cdot & \cdot & \cdot & c_{6} \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.94\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  2 \\
     2 &  0 & -1 &  0 & -1 \\
     0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 \\
    -2 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{3} \\  - v_{3}   +  2  v_{1}   \\ v_{2} \\ v_{3} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{3} &  - c_{3}   +  2  c_{1}   & c_{2} & c_{3} \\
    \cdot & c_{6} &  - c_{6}   +  2  c_{3}   & c_{5} & c_{6} \\
    \cdot & \cdot & c_{6}  -4  c_{3}   +  4  c_{1}   &  - c_{5}   +  2  c_{2}   &  - c_{6}   +  2  c_{3}   \\
    \cdot & \cdot & \cdot & c_{4} & c_{5} \\
    \cdot & \cdot & \cdot & \cdot & c_{6} \\
  \end{bmatrix}
$
}



==> m5_ps_not45_short.tex <==
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -2 &  0 &  0 \\
     0 &  2 &  0 & -2 &  0 \\
     0 &  0 &  2 &  0 & -2 \\
    -1 &  0 &  0 &  2 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v  \\ v \\  2  v  \\ v \\  2  v  \end{bmatrix}
  \begin{bmatrix}
     4  c  &  2  c  &  4  c  &  2  c  &  4  c  \\
    \cdot & c &  2  c  & c &  2  c  \\
    \cdot & \cdot &  4  c  &  2  c  &  4  c  \\
    \cdot & \cdot & \cdot & c &  2  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -2 &  0 &  0 \\
     0 &  2 &  0 & -2 &  0 \\
     0 &  0 &  2 &  0 & -1 \\
    -1 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\ v \\ v \\  2  v  \end{bmatrix}
  \begin{bmatrix}
    c & c & c & c &  2  c  \\
    \cdot & c & c & c &  2  c  \\
    \cdot & \cdot & c & c &  2  c  \\
    \cdot & \cdot & \cdot & c &  2  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -2 &  0 &  0 \\
     0 &  2 &  0 & -1 &  0 \\
     0 &  0 &  1 &  0 & -2 \\
    -1 &  0 &  0 &  2 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  4  v  \\ v \\  4  v  \\  2  v  \\  2  v  \end{bmatrix}
  \begin{bmatrix}
     16  c  &  4  c  &  16  c  &  8  c  &  8  c  \\
    \cdot & c &  4  c  &  2  c  &  2  c  \\
    \cdot & \cdot &  16  c  &  8  c  &  8  c  \\
    \cdot & \cdot & \cdot &  4  c  &  4  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -2 &  0 &  0 \\
     0 &  2 &  0 & -1 &  0 \\
     0 &  0 &  1 &  0 & -1 \\
    -1 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v  \\ v \\  2  v  \\  2  v  \\  2  v  \end{bmatrix}
  \begin{bmatrix}
     4  c  &  2  c  &  4  c  &  4  c  &  4  c  \\
    \cdot & c &  2  c  &  2  c  &  2  c  \\
    \cdot & \cdot &  4  c  &  4  c  &  4  c  \\
    \cdot & \cdot & \cdot &  4  c  &  4  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -2 &  0 &  0 \\
     0 &  2 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{1} \\ v_{2} \\ v_{3} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{4} & c_{2} & c_{4} & c_{5} &  2  c_{2}  \\
    \cdot & c_{1} & c_{2} & c_{3} &  2  c_{1}  \\
    \cdot & \cdot & c_{4} & c_{5} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & c_{6} &  2  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 & -1 \\
     0 &  1 &  0 & -1 &  0 \\
     0 &  1 &  1 &  0 & -1 \\
    -1 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v  \\ v \\ v \\ v \\  2  v  \end{bmatrix}
  \begin{bmatrix}
     4  c  &  2  c  &  2  c  &  2  c  &  4  c  \\
    \cdot & c & c & c &  2  c  \\
    \cdot & \cdot & c & c &  2  c  \\
    \cdot & \cdot & \cdot & c &  2  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 & -1 \\
     0 &  1 &  0 & -1 &  1 \\
     0 &  1 &  1 &  0 & -1 \\
    -1 &  1 & -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  3  v  \\ v \\ v \\  3  v  \\  2  v  \end{bmatrix}
  \begin{bmatrix}
     9  c  &  3  c  &  3  c  &  9  c  &  6  c  \\
    \cdot & c & c &  3  c  &  2  c  \\
    \cdot & \cdot & c &  3  c  &  2  c  \\
    \cdot & \cdot & \cdot &  9  c  &  6  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 &  0 \\
     0 &  1 &  0 & -1 &  0 \\
     0 &  1 &  1 &  0 & -2 \\
    -1 &  0 &  0 &  2 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v  \\ v \\  3  v  \\ v \\  2  v  \end{bmatrix}
  \begin{bmatrix}
     4  c  &  2  c  &  6  c  &  2  c  &  4  c  \\
    \cdot & c &  3  c  & c &  2  c  \\
    \cdot & \cdot &  9  c  &  3  c  &  6  c  \\
    \cdot & \cdot & \cdot & c &  2  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 &  0 \\
     0 &  1 &  0 & -1 &  0 \\
     0 &  1 &  1 &  0 & -1 \\
    -1 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\ v \\ v \\  2  v  \end{bmatrix}
  \begin{bmatrix}
    c & c & c & c &  2  c  \\
    \cdot & c & c & c &  2  c  \\
    \cdot & \cdot & c & c &  2  c  \\
    \cdot & \cdot & \cdot & c &  2  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 &  0 \\
     0 &  1 &  0 & -1 &  1 \\
     0 &  1 &  1 &  0 & -2 \\
    -1 &  0 & -1 &  2 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  3  v  \\ v \\  3  v  \\  3  v  \\  2  v  \end{bmatrix}
  \begin{bmatrix}
     9  c  &  3  c  &  9  c  &  9  c  &  6  c  \\
    \cdot & c &  3  c  &  3  c  &  2  c  \\
    \cdot & \cdot &  9  c  &  9  c  &  6  c  \\
    \cdot & \cdot & \cdot &  9  c  &  6  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 &  0 \\
     0 &  1 &  0 & -1 &  1 \\
     0 &  1 &  1 &  0 & -1 \\
    -1 &  0 & -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v  \\ v \\ v \\  3  v  \\  2  v  \end{bmatrix}
  \begin{bmatrix}
     4  c  &  2  c  &  2  c  &  6  c  &  4  c  \\
    \cdot & c & c &  3  c  &  2  c  \\
    \cdot & \cdot & c &  3  c  &  2  c  \\
    \cdot & \cdot & \cdot &  9  c  &  6  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 & -1 \\
     0 &  1 &  0 & -2 &  0 \\
     0 &  0 &  2 &  0 & -1 \\
    -1 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  3  v  \\  2  v  \\  2  v  \\ v \\  4  v  \end{bmatrix}
  \begin{bmatrix}
     9  c  &  6  c  &  6  c  &  3  c  &  12  c  \\
    \cdot &  4  c  &  4  c  &  2  c  &  8  c  \\
    \cdot & \cdot &  4  c  &  2  c  &  8  c  \\
    \cdot & \cdot & \cdot & c &  4  c  \\
    \cdot & \cdot & \cdot & \cdot &  16  c  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 & -1 \\
     0 &  1 &  0 & -2 &  1 \\
     0 &  0 &  2 &  0 & -1 \\
    -1 &  1 & -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} \frac{ 3 }{ 2 } v  \\ v \\ v \\ \frac{ 3 }{ 2 } v  \\  2  v  \end{bmatrix}
  \begin{bmatrix}
    \frac{ 9 }{ 4 } c  & \frac{ 3 }{ 2 } c  & \frac{ 3 }{ 2 } c  & \frac{ 9 }{ 4 } c  &  3  c  \\
    \cdot & c & c & \frac{ 3 }{ 2 } c  &  2  c  \\
    \cdot & \cdot & c & \frac{ 3 }{ 2 } c  &  2  c  \\
    \cdot & \cdot & \cdot & \frac{ 9 }{ 4 } c  &  3  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 & -1 \\
     0 &  1 &  0 & -1 &  0 \\
     0 &  0 &  1 &  0 & -1 \\
    -1 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v  \\ v \\  2  v  \\ v \\  2  v  \end{bmatrix}
  \begin{bmatrix}
     4  c  &  2  c  &  4  c  &  2  c  &  4  c  \\
    \cdot & c &  2  c  & c &  2  c  \\
    \cdot & \cdot &  4  c  &  2  c  &  4  c  \\
    \cdot & \cdot & \cdot & c &  2  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 & -1 \\
     0 &  1 &  0 & -1 &  1 \\
     0 &  0 &  1 &  0 & -1 \\
    -1 &  1 & -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v  \\ v \\  2  v  \\  3  v  \\  2  v  \end{bmatrix}
  \begin{bmatrix}
     4  c  &  2  c  &  4  c  &  6  c  &  4  c  \\
    \cdot & c &  2  c  &  3  c  &  2  c  \\
    \cdot & \cdot &  4  c  &  6  c  &  4  c  \\
    \cdot & \cdot & \cdot &  9  c  &  6  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 & -1 \\
     0 &  1 &  0 &  1 & -1 \\
     0 &  0 & -1 &  0 &  1 \\
    -1 &  1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v  \\ v \\  2  v  \\ v \\  2  v  \end{bmatrix}
  \begin{bmatrix}
     4  c  &  2  c  &  4  c  &  2  c  &  4  c  \\
    \cdot & c &  2  c  & c &  2  c  \\
    \cdot & \cdot &  4  c  &  2  c  &  4  c  \\
    \cdot & \cdot & \cdot & c &  2  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 \\
     0 &  1 &  0 & -2 &  0 \\
     0 &  0 &  2 &  0 & -1 \\
    -1 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\  2  v  \\  2  v  \\ v \\  4  v  \end{bmatrix}
  \begin{bmatrix}
    c &  2  c  &  2  c  & c &  4  c  \\
    \cdot &  4  c  &  4  c  &  2  c  &  8  c  \\
    \cdot & \cdot &  4  c  &  2  c  &  8  c  \\
    \cdot & \cdot & \cdot & c &  4  c  \\
    \cdot & \cdot & \cdot & \cdot &  16  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 \\
     0 &  1 &  0 & -2 &  1 \\
     0 &  0 &  2 &  0 & -2 \\
    -1 &  0 & -1 &  2 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\  2  v  \\ \frac{ 3 }{ 2 } v  \\  2  v  \end{bmatrix}
  \begin{bmatrix}
    c & c &  2  c  & \frac{ 3 }{ 2 } c  &  2  c  \\
    \cdot & c &  2  c  & \frac{ 3 }{ 2 } c  &  2  c  \\
    \cdot & \cdot &  4  c  &  3  c  &  4  c  \\
    \cdot & \cdot & \cdot & \frac{ 9 }{ 4 } c  &  3  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 \\
     0 &  1 &  0 & -1 &  0 \\
     0 &  0 &  1 &  0 & -1 \\
    -1 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\  2  v  \\ v \\  2  v  \end{bmatrix}
  \begin{bmatrix}
    c & c &  2  c  & c &  2  c  \\
    \cdot & c &  2  c  & c &  2  c  \\
    \cdot & \cdot &  4  c  &  2  c  &  4  c  \\
    \cdot & \cdot & \cdot & c &  2  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 \\
     0 &  1 &  0 & -1 &  1 \\
     0 &  0 &  1 &  0 & -1 \\
    -1 &  0 & -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\  2  v  \\  3  v  \\  2  v  \end{bmatrix}
  \begin{bmatrix}
    c & c &  2  c  &  3  c  &  2  c  \\
    \cdot & c &  2  c  &  3  c  &  2  c  \\
    \cdot & \cdot &  4  c  &  6  c  &  4  c  \\
    \cdot & \cdot & \cdot &  9  c  &  6  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 \\
     0 &  1 &  0 &  1 & -2 \\
     0 &  0 & -1 &  0 &  1 \\
    -1 &  0 &  2 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\  2  v  \\  3  v  \\  2  v  \end{bmatrix}
  \begin{bmatrix}
    c & c &  2  c  &  3  c  &  2  c  \\
    \cdot & c &  2  c  &  3  c  &  2  c  \\
    \cdot & \cdot &  4  c  &  6  c  &  4  c  \\
    \cdot & \cdot & \cdot &  9  c  &  6  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 \\
     0 &  1 &  0 &  1 & -1 \\
     0 &  0 & -1 &  0 &  1 \\
    -1 &  0 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\  2  v  \\ v \\  2  v  \end{bmatrix}
  \begin{bmatrix}
    c & c &  2  c  & c &  2  c  \\
    \cdot & c &  2  c  & c &  2  c  \\
    \cdot & \cdot &  4  c  &  2  c  &  4  c  \\
    \cdot & \cdot & \cdot & c &  2  c  \\
    \cdot & \cdot & \cdot & \cdot &  4  c  \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 \\
     2 &  0 &  0 &  0 & -2 \\
     0 &  0 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 &  0 \\
    -1 &  2 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{1}  \\ v_{1} \\ v_{2} \\ v_{3} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     4  c_{1}  &  2  c_{1}  &  2  c_{2}  &  2  c_{3}  &  4  c_{1}  \\
    \cdot & c_{1} & c_{2} & c_{3} &  2  c_{1}  \\
    \cdot & \cdot & c_{4} & c_{5} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & c_{6} &  2  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  2 \\
     2 &  0 & -2 &  0 &  0 \\
     0 &  2 &  0 & -2 &  0 \\
     0 &  0 &  2 &  0 & -2 \\
    -2 &  0 &  0 &  2 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\ v \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
    c & c & c & c & c \\
    \cdot & c & c & c & c \\
    \cdot & \cdot & c & c & c \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  2 \\
     2 &  0 & -2 &  0 &  0 \\
     0 &  2 &  0 & -1 & -1 \\
     0 &  0 &  1 &  0 & -1 \\
    -2 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\ v \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
    c & c & c & c & c \\
    \cdot & c & c & c & c \\
    \cdot & \cdot & c & c & c \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  2 \\
     2 &  0 & -2 &  0 &  0 \\
     0 &  2 &  0 &  0 & -2 \\
     0 &  0 &  0 &  0 &  0 \\
    -2 &  0 &  2 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{3} \\ v_{1} \\ v_{2} \\ v_{3} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{3} & c_{1} & c_{2} & c_{3} \\
    \cdot & c_{6} & c_{3} & c_{5} & c_{6} \\
    \cdot & \cdot & c_{1} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & c_{4} & c_{5} \\
    \cdot & \cdot & \cdot & \cdot & c_{6} \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  2 \\
     2 &  0 & -1 &  0 & -1 \\
     0 &  1 &  0 & -1 &  0 \\
     0 &  0 &  1 &  0 & -1 \\
    -2 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\ v \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
    c & c & c & c & c \\
    \cdot & c & c & c & c \\
    \cdot & \cdot & c & c & c \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  2 \\
     2 &  0 &  0 &  0 & -2 \\
     0 &  0 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 &  0 \\
    -2 &  2 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{3} \\ v_{3} \\ v_{1} \\ v_{2} \\ v_{3} \end{bmatrix}
  \begin{bmatrix}
    c_{6} & c_{6} & c_{3} & c_{5} & c_{6} \\
    \cdot & c_{6} & c_{3} & c_{5} & c_{6} \\
    \cdot & \cdot & c_{1} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & c_{4} & c_{5} \\
    \cdot & \cdot & \cdot & \cdot & c_{6} \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 & -1 \\
     0 &  1 &  0 & -1 &  0 \\
    -1 &  1 &  1 &  0 & -1 \\
    -1 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v  \\ v \\  2  v  \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
     4  c  &  2  c  &  4  c  &  2  c  &  2  c  \\
    \cdot & c &  2  c  & c & c \\
    \cdot & \cdot &  4  c  &  2  c  &  2  c  \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 & -1 \\
     0 &  1 &  0 & -1 &  1 \\
    -1 &  1 &  1 &  0 & -1 \\
    -1 &  1 & -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  3  v  \\  2  v  \\  2  v  \\  3  v  \\ v \end{bmatrix}
  \begin{bmatrix}
     9  c  &  6  c  &  6  c  &  9  c  &  3  c  \\
    \cdot &  4  c  &  4  c  &  6  c  &  2  c  \\
    \cdot & \cdot &  4  c  &  6  c  &  2  c  \\
    \cdot & \cdot & \cdot &  9  c  &  3  c  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 &  0 \\
     0 &  1 &  0 & -1 &  0 \\
    -1 &  1 &  1 &  0 & -1 \\
    -1 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\ v \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
    c & c & c & c & c \\
    \cdot & c & c & c & c \\
    \cdot & \cdot & c & c & c \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 &  0 \\
     0 &  1 &  0 & -1 &  1 \\
    -1 &  1 &  1 &  0 & -1 \\
    -1 &  0 & -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v  \\  2  v  \\ v \\  3  v  \\ v \end{bmatrix}
  \begin{bmatrix}
     4  c  &  4  c  &  2  c  &  6  c  &  2  c  \\
    \cdot &  4  c  &  2  c  &  6  c  &  2  c  \\
    \cdot & \cdot & c &  3  c  & c \\
    \cdot & \cdot & \cdot &  9  c  &  3  c  \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 &  0 \\
     0 &  1 &  0 &  0 & -1 \\
    -1 &  1 &  0 &  0 &  0 \\
    -1 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\ v \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
    c & c & c & c & c \\
    \cdot & c & c & c & c \\
    \cdot & \cdot & c & c & c \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 &  0 \\
     0 &  1 &  0 &  0 & -1 \\
    -1 &  1 &  0 &  0 &  1 \\
    -1 &  0 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v  \\ v \\  3  v  \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
     4  c  &  2  c  &  6  c  &  2  c  &  2  c  \\
    \cdot & c &  3  c  & c & c \\
    \cdot & \cdot &  9  c  &  3  c  &  3  c  \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}

\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 &  0 \\
     0 &  1 &  0 &  1 & -2 \\
    -1 &  1 & -1 &  0 &  1 \\
    -1 &  0 &  2 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v \\ v \\ v \\ v \\ v \end{bmatrix}
  \begin{bmatrix}
    c & c & c & c & c \\
    \cdot & c & c & c & c \\
    \cdot & \cdot & c & c & c \\
    \cdot & \cdot & \cdot & c & c \\
    \cdot & \cdot & \cdot & \cdot & c \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.06\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.43\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 &  0 \\
     0 &  1 &  0 &  1 & -1 \\
    -1 &  1 & -1 &  0 &  1 \\
    -1 &  0 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v  \\  2  v  \\  3  v  \\ v \\  3  v  \end{bmatrix}
  \begin{bmatrix}
     2  c  &  2  c  &  3  c  & c &  3  c  \\
    \cdot &  2  c  &  3  c  & c &  3  c  \\
    \cdot & \cdot & \frac{ 9 }{ 2 } c  & \frac{ 3 }{ 2 } c  & \frac{ 9 }{ 2 } c  \\
    \cdot & \cdot & \cdot & \frac{ 1 }{ 2 } c  & \frac{ 3 }{ 2 } c  \\
    \cdot & \cdot & \cdot & \cdot & \frac{ 9 }{ 2 } c  \\
  \end{bmatrix}
$
}



==> m6_notps_short.tex <==
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -2 &  0 &  0 &  0 \\
     0 &  2 &  0 & -1 & -1 & -1 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
    -1 &  0 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{1}  \\ v_{1} \\  2  v_{1}  \\  - v_{2}  \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     4  c_{1}  &  2  c_{1}  &  4  c_{1}  &  -2  c_{2}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & c_{1} &  2  c_{1}  &  - c_{2}  & c_{2} &  2  c_{1}  \\
    \cdot & \cdot &  4  c_{1}  &  -2  c_{2}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & \cdot & \cdot & c_{3} &  - c_{3}  &  -2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -2 &  0 &  0 &  0 \\
     0 &  2 &  0 & -1 &  0 & -1 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{1}  \\ v_{1} \\  2  v_{1}  \\  0  \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     4  c_{1}  &  2  c_{1}  &  4  c_{1}  &  0  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & c_{1} &  2  c_{1}  &  0  & c_{2} &  2  c_{1}  \\
    \cdot & \cdot &  4  c_{1}  &  0  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -2 &  0 &  0 &  0 \\
     0 &  2 &  0 &  0 &  0 & -2 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  2 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  0  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 &  0 & -1 \\
     0 &  1 &  0 & -1 &  0 & -1 \\
     0 &  1 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v_{1}  \\  - v_{1}  \\  - v_{1}  \\ v_{1} \\ v_{2} \\  -2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{1} & c_{1} &  - c_{1}  &  - c_{2}  &  2  c_{1}  \\
    \cdot & c_{1} & c_{1} &  - c_{1}  &  - c_{2}  &  2  c_{1}  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  2  c_{1}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  -2  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  -2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 &  0 & -1 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  - v_{1}  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 &  0 &  0 \\
     0 &  1 &  0 & -1 &  0 & -1 \\
     0 &  1 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  - v_{1}  \\  - v_{1}  \\ v_{1} \\ v_{2} \\  -2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{1} & c_{1} &  - c_{1}  &  - c_{2}  &  2  c_{1}  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  2  c_{1}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  -2  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  -2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 &  0 &  0 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  - v_{1}  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 & -1 \\
     0 &  1 &  0 & -1 &  0 & -1 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  -2  v_{1}  \\  - v_{1}  \\  -2  v_{1}  \\ v_{1} \\ v_{2} \\  -2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     4  c_{1}  &  2  c_{1}  &  4  c_{1}  &  -2  c_{1}  &  -2  c_{2}  &  4  c_{1}  \\
    \cdot & c_{1} &  2  c_{1}  &  - c_{1}  &  - c_{2}  &  2  c_{1}  \\
    \cdot & \cdot &  4  c_{1}  &  -2  c_{1}  &  -2  c_{2}  &  4  c_{1}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  -2  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  -2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  0  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 &  0 \\
     0 &  1 &  0 & -1 &  0 & -1 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v_{1}  \\  - v_{1}  \\  -2  v_{1}  \\ v_{1} \\ v_{2} \\  -2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{1} &  2  c_{1}  &  - c_{1}  &  - c_{2}  &  2  c_{1}  \\
    \cdot & c_{1} &  2  c_{1}  &  - c_{1}  &  - c_{2}  &  2  c_{1}  \\
    \cdot & \cdot &  4  c_{1}  &  -2  c_{1}  &  -2  c_{2}  &  4  c_{1}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  -2  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  -2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 &  0 \\
     0 &  1 &  0 &  0 &  0 & -2 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  2 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  0  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 &  0 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  1 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  0  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 & -1 & -1 & -1 & -1 \\
     0 &  1 &  0 & -1 & -1 & -1 \\
     0 &  1 &  1 &  0 &  0 & -1 \\
     0 &  1 &  1 &  0 &  0 & -1 \\
    -2 &  1 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  2  v_{1}  \\  0  \\  - v_{2}  \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  2  c_{1}  &  0  &  - c_{2}  & c_{2} &  2  c_{1}  \\
    \cdot &  4  c_{1}  &  0  &  -2  c_{2}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{3} &  - c_{3}  &  -2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 & -1 & -1 & -1 & -1 \\
     0 &  1 &  0 & -1 &  0 &  0 \\
     0 &  1 &  1 &  0 &  1 & -1 \\
     0 &  1 &  0 & -1 &  0 &  0 \\
    -2 &  1 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\  - v_{1}  \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} &  - c_{2}  & c_{3} & c_{2} & c_{3} \\
    \cdot & c_{3} &  - c_{2}  & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & c_{1} &  - c_{2}  &  - c_{1}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 & -1 & -1 & -1 &  0 \\
     0 &  1 &  0 & -1 & -1 & -1 \\
     0 &  1 &  1 &  0 & -1 & -1 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -2 &  0 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\  2  v_{1}  \\  -2  v_{1}  \\  2  v_{1}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    \frac{ 1 }{ 4 } c_{2}  & \frac{ 1 }{ 2 } c_{3}  & \frac{ 1 }{ 2 } c_{2}  & \frac{ -1 }{ 2 } c_{2}  & \frac{ 1 }{ 2 } c_{2}  & \frac{ 1 }{ 2 } c_{3}  \\
    \cdot & c_{1} & c_{3} &  - c_{3}  & c_{3} & c_{1} \\
    \cdot & \cdot & c_{2} &  - c_{2}  & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & c_{2} &  - c_{2}  &  - c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{1} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 & -1 & -1 & -1 &  0 \\
     0 &  1 &  0 & -1 & -1 & -1 \\
     0 &  1 &  1 &  0 &  0 & -1 \\
     0 &  1 &  1 &  0 &  0 & -1 \\
    -2 &  0 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{2} \\  0  \\  - v_{1}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} &  0  &  - c_{2}  & c_{2} & c_{3} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 & -1 & -1 & -1 &  0 \\
     0 &  1 &  0 & -1 &  0 & -1 \\
     0 &  1 &  1 &  0 & -1 & -1 \\
     0 &  1 &  0 &  1 &  0 & -1 \\
    -2 &  0 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\ v_{1} \\  0  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{2} & c_{3} & c_{2} &  0  & c_{2} & c_{3} \\
    \cdot & c_{1} & c_{3} &  0  & c_{3} & c_{1} \\
    \cdot & \cdot & c_{2} &  0  & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{1} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 & -1 & -1 & -1 &  0 \\
     0 &  1 &  0 & -1 &  0 & -1 \\
     0 &  1 &  1 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
    -2 &  0 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\  0  \\  0  \\  2  v_{1}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    \frac{ 1 }{ 2 } c_{1}  & \frac{ 1 }{ 2 } c_{3}  &  0  &  0  & c_{1} & \frac{ 1 }{ 2 } c_{3}  \\
    \cdot & c_{2} &  0  &  0  & c_{3} & c_{2} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot &  2  c_{1}  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 & -1 & -1 &  0 & -1 \\
     0 &  1 &  0 & -1 &  0 & -1 \\
     0 &  1 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -2 &  1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  2  v_{1}  \\  0  \\  0  \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  2  c_{1}  &  0  &  0  & c_{2} &  2  c_{1}  \\
    \cdot &  4  c_{1}  &  0  &  0  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 & -1 & -1 &  0 & -1 \\
     0 &  1 &  0 & -1 &  0 &  0 \\
     0 &  1 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -2 &  1 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\  0  \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} &  0  & c_{3} & c_{2} & c_{3} \\
    \cdot & c_{3} &  0  & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 & -1 & -1 &  0 &  0 \\
     0 &  1 &  0 & -1 & -1 & -1 \\
     0 &  1 &  1 &  0 &  1 & -1 \\
     0 &  0 &  1 & -1 &  0 &  0 \\
    -2 &  0 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v_{1}  \\ v_{2} \\  - v_{1}  \\  - v_{1}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{2} & c_{3} & c_{2} & c_{2} &  - c_{2}  & c_{3} \\
    \cdot & c_{1} & c_{3} & c_{3} &  - c_{3}  & c_{1} \\
    \cdot & \cdot & c_{2} & c_{2} &  - c_{2}  & c_{3} \\
    \cdot & \cdot & \cdot & c_{2} &  - c_{2}  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{2} &  - c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{1} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 & -1 & -1 &  0 &  0 \\
     0 &  1 &  0 & -1 &  0 & -1 \\
     0 &  1 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -2 &  0 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{2} \\  0  \\  0  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} &  0  &  0  & c_{2} & c_{3} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 & -1 & -1 &  0 &  0 \\
     0 &  1 &  0 &  0 & -1 & -1 \\
     0 &  1 &  0 &  0 &  1 & -1 \\
     0 &  0 &  1 & -1 &  0 &  0 \\
    -2 &  0 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\ v_{1} \\ v_{1} \\  0  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{2} & c_{3} & c_{2} & c_{2} &  0  & c_{3} \\
    \cdot & c_{1} & c_{3} & c_{3} &  0  & c_{1} \\
    \cdot & \cdot & c_{2} & c_{2} &  0  & c_{3} \\
    \cdot & \cdot & \cdot & c_{2} &  0  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{1} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 & -1 & -1 \\
     0 &  1 &  0 &  0 & -1 & -1 \\
     0 &  1 &  0 &  0 & -1 & -1 \\
    -1 &  1 &  1 &  1 &  0 &  0 \\
    -1 &  1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  - v_{1}  \\ v_{1} \\  - v_{2}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{1} &  - c_{1}  & c_{2} &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} &  - c_{2}  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  - c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 & -1 & -1 \\
     0 &  1 &  0 &  0 & -1 &  0 \\
     0 &  1 &  0 &  0 & -1 &  0 \\
    -1 &  1 &  1 &  1 &  0 &  0 \\
    -1 &  1 &  0 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\  - v_{1}  \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} &  - c_{2}  & c_{2} & c_{3} & c_{3} \\
    \cdot & c_{3} &  - c_{2}  & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 & -1 & -1 \\
     0 &  1 &  0 &  0 & -1 &  1 \\
     0 &  1 &  0 &  0 & -1 &  1 \\
    -1 &  1 &  1 &  1 &  0 &  0 \\
    -1 &  1 & -1 & -1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{2}  \\  2  v_{2}  \\  - v_{1}  \\ v_{1} \\  3  v_{2}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     4  c_{3}  &  4  c_{3}  &  -2  c_{2}  &  2  c_{2}  &  6  c_{3}  &  2  c_{3}  \\
    \cdot &  4  c_{3}  &  -2  c_{2}  &  2  c_{2}  &  6  c_{3}  &  2  c_{3}  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  -3  c_{2}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} &  3  c_{2}  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot &  9  c_{3}  &  3  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 &  0 &  0 \\
     0 &  1 &  0 &  0 & -1 & -1 \\
     0 &  1 &  0 &  0 & -1 & -1 \\
    -1 &  0 &  1 &  1 &  0 &  0 \\
    -1 &  0 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  - v_{1}  \\ v_{1} \\  - v_{2}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{1} &  - c_{1}  & c_{2} &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} &  - c_{2}  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  - c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 &  0 & -1 & -1 \\
     0 &  1 &  0 &  0 & -1 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 & -1 \\
    -1 &  1 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  0  \\  2  v_{2}  \\ v_{1} \\  - v_{2}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  0  &  2  c_{3}  & c_{2} &  - c_{3}  & c_{3} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  4  c_{3}  &  2  c_{2}  &  -2  c_{3}  &  2  c_{3}  \\
    \cdot & \cdot & \cdot & c_{1} &  - c_{2}  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  - c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 &  0 & -1 & -1 \\
     0 &  1 &  0 &  0 & -1 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  0  \\ v_{1} \\  - v_{2}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} &  - c_{2}  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  - c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 &  0 & -1 & -1 \\
     0 &  1 &  0 &  0 & -1 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 &  0 \\
    -1 &  1 &  0 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\  0  \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} &  0  & c_{2} & c_{3} & c_{3} \\
    \cdot & c_{3} &  0  & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 &  0 & -1 & -1 \\
     0 &  1 &  0 &  0 & -1 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 &  1 \\
    -1 &  1 &  0 &  0 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{2} \\  -2  v_{2}  \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} &  -2  c_{3}  & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot &  4  c_{3}  &  -2  c_{2}  &  -2  c_{3}  &  -2  c_{3}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 &  0 & -1 & -1 \\
     0 &  1 &  0 &  0 & -1 &  1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 &  0 \\
    -1 &  1 & -1 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{2}  \\  2  v_{2}  \\  0  \\ v_{1} \\  3  v_{2}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     4  c_{3}  &  4  c_{3}  &  0  &  2  c_{2}  &  6  c_{3}  &  2  c_{3}  \\
    \cdot &  4  c_{3}  &  0  &  2  c_{2}  &  6  c_{3}  &  2  c_{3}  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} &  3  c_{2}  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot &  9  c_{3}  &  3  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 &  0 & -1 & -1 \\
     0 &  1 &  0 &  0 & -1 &  1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 &  1 \\
    -1 &  1 & -1 &  0 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  2  v_{2}  \\  -2  v_{2}  \\ v_{1} \\  3  v_{2}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  2  c_{3}  &  -2  c_{3}  & c_{2} &  3  c_{3}  & c_{3} \\
    \cdot &  4  c_{3}  &  -4  c_{3}  &  2  c_{2}  &  6  c_{3}  &  2  c_{3}  \\
    \cdot & \cdot &  4  c_{3}  &  -2  c_{2}  &  -6  c_{3}  &  -2  c_{3}  \\
    \cdot & \cdot & \cdot & c_{1} &  3  c_{2}  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot &  9  c_{3}  &  3  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 &  0 & -1 &  0 \\
     0 &  1 &  0 &  0 & -1 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 & -1 \\
    -1 &  0 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\ v_{2} \\ v_{1} \\  - v_{2}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{3} & c_{2} &  - c_{3}  & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} &  - c_{2}  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  - c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 &  0 & -1 &  0 \\
     0 &  1 &  0 &  0 & -1 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 &  0 \\
    -1 &  0 &  1 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v_{2}  \\  0  \\  - v_{2}  \\ v_{1} \\  - v_{2}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  0  & c_{3} &  - c_{2}  & c_{3} &  - c_{3}  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{3} &  - c_{2}  & c_{3} &  - c_{3}  \\
    \cdot & \cdot & \cdot & c_{1} &  - c_{2}  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  - c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 &  0 & -1 &  0 \\
     0 &  1 &  0 &  0 & -1 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 &  1 \\
    -1 &  0 &  1 &  0 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  -2  v_{2}  \\  0  \\  -3  v_{2}  \\ v_{1} \\  - v_{2}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     4  c_{3}  &  0  &  6  c_{3}  &  -2  c_{2}  &  2  c_{3}  &  -2  c_{3}  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  9  c_{3}  &  -3  c_{2}  &  3  c_{3}  &  -3  c_{3}  \\
    \cdot & \cdot & \cdot & c_{1} &  - c_{2}  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  - c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 &  0 &  0 & -1 & -1 \\
     0 &  0 &  0 &  0 & -1 &  1 \\
     0 &  0 &  0 &  0 & -1 &  1 \\
    -1 &  1 &  1 &  1 &  0 &  0 \\
    -1 &  1 & -1 & -1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\  - v_{1}  \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} &  - c_{2}  & c_{2} & c_{3} & c_{3} \\
    \cdot & c_{3} &  - c_{2}  & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 &  0 &  0 & -1 & -1 \\
     0 &  0 &  0 &  0 & -1 &  1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 &  0 \\
    -1 &  1 & -1 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\  0  \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} &  0  & c_{2} & c_{3} & c_{3} \\
    \cdot & c_{3} &  0  & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 &  0 &  0 & -1 & -1 \\
     0 &  0 &  0 &  0 & -1 &  1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 &  1 \\
    -1 &  1 & -1 &  0 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\  - v_{2}  \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} &  - c_{3}  & c_{2} & c_{3} & c_{3} \\
    \cdot & c_{3} &  - c_{3}  & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot & c_{3} &  - c_{2}  &  - c_{3}  &  - c_{3}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 &  0 &  0 & -1 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  0 &  0 &  0 & -1 \\
    -1 &  1 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\ v_{1} \\ v_{2} \\  0  \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{1} & c_{2} &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{3} &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 &  1 \\
     2 &  0 &  0 & -1 & -1 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  0 &  0 & -1 & -1 \\
    -1 &  1 &  0 &  1 &  0 & -1 \\
    -1 &  1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{1} \\ v_{2} \\  2  v_{1}  \\  -2  v_{1}  \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{1} & c_{2} &  2  c_{1}  &  -2  c_{1}  &  2  c_{1}  \\
    \cdot & c_{1} & c_{2} &  2  c_{1}  &  -2  c_{1}  &  2  c_{1}  \\
    \cdot & \cdot & c_{3} &  2  c_{2}  &  -2  c_{2}  &  2  c_{2}  \\
    \cdot & \cdot & \cdot &  4  c_{1}  &  -4  c_{1}  &  4  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot &  4  c_{1}  &  -4  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 &  1 \\
     2 &  0 &  0 & -1 & -1 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  0 &  0 & -1 & -1 \\
    -1 &  1 &  0 &  1 &  0 &  0 \\
    -1 &  1 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\ v_{1} \\  0  \\  - v_{2}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{1} &  0  &  - c_{2}  & c_{2} \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  - c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 &  1 \\
     2 &  0 &  0 & -1 & -1 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  0 &  0 & -1 &  0 \\
    -1 &  1 &  0 &  1 &  0 & -1 \\
    -1 &  1 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\ v_{1} \\ v_{2} \\  0  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} & c_{2} & c_{3} &  0  & c_{3} \\
    \cdot & c_{3} & c_{2} & c_{3} &  0  & c_{3} \\
    \cdot & \cdot & c_{1} & c_{2} &  0  & c_{2} \\
    \cdot & \cdot & \cdot & c_{3} &  0  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  1 &  1 &  1 \\
     2 &  0 &  0 & -1 & -1 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  0 &  0 & -1 &  0 \\
    -1 &  1 &  0 &  1 &  0 &  0 \\
    -1 &  1 &  0 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{1} \\ v_{2} \\  0  \\  0  \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{1} & c_{2} &  0  &  0  &  2  c_{1}  \\
    \cdot & c_{1} & c_{2} &  0  &  0  &  2  c_{1}  \\
    \cdot & \cdot & c_{3} &  0  &  0  &  2  c_{2}  \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  1 &  1 &  1 &  1 \\
     2 &  0 & -1 & -1 & -1 & -1 \\
    -1 &  1 &  0 & -1 & -1 &  0 \\
    -1 &  1 &  1 &  0 &  0 & -1 \\
    -1 &  1 &  1 &  0 &  0 & -1 \\
    -1 &  1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\ v_{2} \\  - v_{1}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} & c_{3} &  - c_{2}  & c_{2} & c_{3} \\
    \cdot & c_{3} & c_{3} &  - c_{2}  & c_{2} & c_{3} \\
    \cdot & \cdot & c_{3} &  - c_{2}  & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  1 &  1 &  1 &  1 \\
     2 &  0 & -1 & -1 & -1 & -1 \\
    -1 &  1 &  0 & -1 & -1 &  0 \\
    -1 &  1 &  1 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 &  0 \\
    -1 &  1 &  0 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{1} \\  0  \\  - v_{2}  \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{1} &  0  &  - c_{2}  & c_{2} &  2  c_{1}  \\
    \cdot & c_{1} &  0  &  - c_{2}  & c_{2} &  2  c_{1}  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{3} &  - c_{3}  &  -2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  1 &  1 &  1 &  1 \\
     2 &  0 & -1 & -1 & -1 & -1 \\
    -1 &  1 &  0 & -1 & -1 &  0 \\
    -1 &  1 &  1 &  0 &  0 &  1 \\
    -1 &  1 &  1 &  0 &  0 &  1 \\
    -1 &  1 &  0 & -1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  - v_{2}  \\  - v_{1}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{3} & c_{2} &  - c_{2}  &  - c_{3}  \\
    \cdot & \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 & -1 &  0 \\
     1 &  1 &  0 & -1 & -1 & -1 \\
     1 &  1 &  1 &  0 &  0 & -1 \\
     1 &  1 &  1 &  0 &  0 & -1 \\
    -1 &  0 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{2} \\  0  \\  - v_{1}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} &  0  &  - c_{2}  & c_{2} & c_{3} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 & -1 &  0 \\
     1 &  1 &  0 & -1 &  0 & -1 \\
     1 &  1 &  1 &  0 &  1 & -1 \\
     1 &  1 &  0 & -1 &  0 & -1 \\
    -1 &  0 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{2} \\  - v_{1}  \\  0  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} &  - c_{2}  &  0  & c_{2} & c_{3} \\
    \cdot & \cdot & c_{1} &  0  &  - c_{1}  &  - c_{2}  \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 & -1 &  0 \\
     1 &  1 &  0 & -1 &  0 &  0 \\
     1 &  1 &  1 &  0 &  1 & -1 \\
     1 &  1 &  0 & -1 &  0 &  0 \\
    -1 &  0 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  0  \\  - v_{1}  \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  0  &  - c_{2}  & c_{3} & c_{2} & c_{3} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{1} &  - c_{2}  &  - c_{1}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 & -1 &  0 \\
     1 &  1 &  0 & -1 &  0 &  1 \\
     1 &  1 &  1 &  0 &  1 & -1 \\
     1 &  1 &  0 & -1 &  0 &  1 \\
    -1 &  0 & -1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{2}  \\  - v_{2}  \\  - v_{1}  \\  2  v_{2}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     4  c_{3}  &  -2  c_{3}  &  -2  c_{2}  &  4  c_{3}  &  2  c_{2}  &  2  c_{3}  \\
    \cdot & c_{3} & c_{2} &  -2  c_{3}  &  - c_{2}  &  - c_{3}  \\
    \cdot & \cdot & c_{1} &  -2  c_{2}  &  - c_{1}  &  - c_{2}  \\
    \cdot & \cdot & \cdot &  4  c_{3}  &  2  c_{2}  &  2  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 & -1 &  1 \\
     1 &  1 &  0 & -1 & -1 &  0 \\
     1 &  1 &  1 &  0 &  0 & -1 \\
     1 &  1 &  1 &  0 &  0 & -1 \\
    -1 & -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\ v_{2} \\  - v_{1}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{3} &  - c_{2}  & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 & -1 &  1 \\
     1 &  1 &  0 & -1 &  0 &  1 \\
     1 &  1 &  1 &  0 & -1 &  0 \\
     1 &  1 &  0 &  1 &  0 & -1 \\
    -1 & -1 & -1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{1}  \\  -2  v_{1}  \\ v_{1} \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     -2  c_{1}  &  2  c_{1}  &  - c_{1}  &  - c_{2}  &  - c_{1}  &  - c_{2}  \\
    \cdot &  -2  c_{1}  & c_{1} & c_{2} & c_{1} & c_{2} \\
    \cdot & \cdot & \frac{ -1 }{ 2 } c_{1}  & \frac{ -1 }{ 2 } c_{2}  & \frac{ -1 }{ 2 } c_{1}  & \frac{ -1 }{ 2 } c_{2}  \\
    \cdot & \cdot & \cdot & c_{3} & \frac{ -1 }{ 2 } c_{2}  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \frac{ -1 }{ 2 } c_{1}  & \frac{ -1 }{ 2 } c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 &  0 & -1 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     1 &  0 &  1 &  1 &  0 & -1 \\
    -1 &  1 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{2}  \\ v_{2} \\  - v_{1}  \\ v_{1} \\ v_{2} \\  2  v_{2}  \end{bmatrix}
  \begin{bmatrix}
     4  c_{1}  &  2  c_{1}  &  2  c_{2}  &  -2  c_{2}  &  2  c_{1}  &  4  c_{1}  \\
    \cdot & c_{1} & c_{2} &  - c_{2}  & c_{1} &  2  c_{1}  \\
    \cdot & \cdot & c_{3} &  - c_{3}  & c_{2} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & c_{3} &  - c_{2}  &  -2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} &  2  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 &  0 & -1 \\
     1 &  1 &  0 &  0 & -1 &  0 \\
     1 &  1 &  0 &  0 & -1 &  0 \\
     1 &  0 &  1 &  1 &  0 & -1 \\
    -1 &  1 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  0  \\  - v_{1}  \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  0  &  - c_{2}  & c_{2} & c_{3} & c_{3} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 &  0 & -1 \\
     1 &  1 &  0 &  0 & -1 &  1 \\
     1 &  1 &  0 &  0 & -1 &  1 \\
     1 &  0 &  1 &  1 &  0 & -1 \\
    -1 &  1 & -1 & -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ \frac{ -1 }{ 2 } v_{2}  \\  - v_{1}  \\ v_{1} \\ \frac{ 3 }{ 2 } v_{2}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     4  c_{1}  &  -2  c_{1}  &  - c_{3}  & c_{3} &  6  c_{1}  &  4  c_{1}  \\
    \cdot & c_{1} & \frac{ 1 }{ 2 } c_{3}  & \frac{ -1 }{ 2 } c_{3}  &  -3  c_{1}  &  -2  c_{1}  \\
    \cdot & \cdot & c_{2} &  - c_{2}  & \frac{ -3 }{ 2 } c_{3}  &  - c_{3}  \\
    \cdot & \cdot & \cdot & c_{2} & \frac{ 3 }{ 2 } c_{3}  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot &  9  c_{1}  &  6  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 &  0 & -1 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     1 &  0 &  0 &  0 &  0 & -1 \\
    -1 &  1 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  0  \\  - v_{1}  \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  0  &  - c_{2}  & c_{2} & c_{3} & c_{3} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 &  0 & -1 \\
     1 &  1 &  0 &  0 &  1 & -1 \\
     1 &  1 &  0 &  0 &  1 & -1 \\
     1 &  0 & -1 & -1 &  0 & -1 \\
    -1 &  1 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  - v_{2}  \\  - v_{1}  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} & c_{2} &  - c_{2}  &  - c_{3}  &  0  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 &  0 &  0 \\
     1 &  1 &  0 & -1 &  0 & -1 \\
     1 &  1 &  1 &  0 &  1 & -1 \\
     1 &  0 &  0 & -1 &  0 &  0 \\
    -1 &  0 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v_{1}  \\ v_{2} \\  0  \\  - v_{1}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  - c_{2}  &  0  & c_{1} &  - c_{1}  &  - c_{2}  \\
    \cdot & c_{3} &  0  &  - c_{2}  & c_{2} & c_{3} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 &  0 &  0 \\
     1 &  1 &  0 &  0 & -1 &  1 \\
     1 &  1 &  0 &  0 &  1 & -1 \\
     1 &  0 &  1 & -1 &  0 &  0 \\
    -1 &  0 & -1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  - v_{1}  \\  0  \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  - c_{1}  &  0  & c_{1} & c_{2} & c_{2} \\
    \cdot & c_{1} &  0  &  - c_{1}  &  - c_{2}  &  - c_{2}  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 &  0 &  1 \\
     1 &  1 &  0 & -1 & -1 &  0 \\
     1 &  1 &  1 &  0 &  1 & -1 \\
     1 &  0 &  1 & -1 &  0 & -1 \\
    -1 & -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  -2  v_{1}  \\ v_{1} \\ v_{2} \\  -2  v_{1}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     -2  c_{2}  & c_{2} & c_{3} &  -2  c_{2}  & c_{2} & c_{3} \\
    \cdot & \frac{ -1 }{ 2 } c_{2}  & \frac{ -1 }{ 2 } c_{3}  & c_{2} & \frac{ -1 }{ 2 } c_{2}  & \frac{ -1 }{ 2 } c_{3}  \\
    \cdot & \cdot & c_{1} & c_{3} & \frac{ -1 }{ 2 } c_{3}  & c_{1} \\
    \cdot & \cdot & \cdot &  -2  c_{2}  & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \frac{ -1 }{ 2 } c_{2}  & \frac{ -1 }{ 2 } c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{1} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 &  0 &  1 \\
     1 &  1 &  0 & -1 &  1 &  1 \\
     1 &  1 &  1 &  0 & -1 &  0 \\
     1 &  0 & -1 &  1 &  0 & -1 \\
    -1 & -1 & -1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{1}  \\  -3  v_{1}  \\  2  v_{1}  \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     2  c_{1}  &  -3  c_{1}  &  2  c_{1}  & c_{2} & c_{1} & c_{2} \\
    \cdot & \frac{ 9 }{ 2 } c_{1}  &  -3  c_{1}  & \frac{ -3 }{ 2 } c_{2}  & \frac{ -3 }{ 2 } c_{1}  & \frac{ -3 }{ 2 } c_{2}  \\
    \cdot & \cdot &  2  c_{1}  & c_{2} & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & c_{3} & \frac{ 1 }{ 2 } c_{2}  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \frac{ 1 }{ 2 } c_{1}  & \frac{ 1 }{ 2 } c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 &  0 &  1 \\
     1 &  1 &  0 &  0 &  1 & -1 \\
     1 &  1 &  0 &  0 &  1 & -1 \\
     1 &  0 & -1 & -1 &  0 &  1 \\
    -1 & -1 &  1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  - v_{2}  \\  - v_{1}  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} & c_{2} &  - c_{2}  &  - c_{3}  &  0  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 &  1 & -1 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     1 & -1 &  1 &  1 &  0 &  0 \\
    -1 &  1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{1} \\  - v_{2}  \\ v_{2} \\ \frac{ 1 }{ 2 } v_{1}  \\ \frac{ 3 }{ 2 } v_{1}  \end{bmatrix}
  \begin{bmatrix}
     4  c_{3}  &  4  c_{3}  &  - c_{1}  & c_{1} &  2  c_{3}  &  6  c_{3}  \\
    \cdot &  4  c_{3}  &  - c_{1}  & c_{1} &  2  c_{3}  &  6  c_{3}  \\
    \cdot & \cdot & c_{2} &  - c_{2}  & \frac{ -1 }{ 2 } c_{1}  & \frac{ -3 }{ 2 } c_{1}  \\
    \cdot & \cdot & \cdot & c_{2} & \frac{ 1 }{ 2 } c_{1}  & \frac{ 3 }{ 2 } c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  3  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  9  c_{3}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 &  1 & -1 \\
     1 &  1 &  0 &  0 & -1 &  0 \\
     1 &  1 &  0 &  0 & -1 &  0 \\
     1 & -1 &  1 &  1 &  0 &  0 \\
    -1 &  1 &  0 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{1} \\  - v_{2}  \\ v_{2} \\  2  v_{1}  \\  3  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{1} &  - c_{2}  & c_{2} &  2  c_{1}  &  3  c_{1}  \\
    \cdot & c_{1} &  - c_{2}  & c_{2} &  2  c_{1}  &  3  c_{1}  \\
    \cdot & \cdot & c_{3} &  - c_{3}  &  -2  c_{2}  &  -3  c_{2}  \\
    \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  &  3  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot &  4  c_{1}  &  6  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  9  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 &  1 & -1 \\
     1 &  1 &  0 &  0 & -1 &  1 \\
     1 &  1 &  0 &  0 & -1 &  1 \\
     1 & -1 &  1 &  1 &  0 &  0 \\
    -1 &  1 & -1 & -1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  - v_{1}  \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 &  1 & -1 \\
     1 &  1 &  0 &  0 & -1 &  1 \\
     1 &  1 &  0 &  0 &  1 & -1 \\
     1 & -1 &  1 & -1 &  0 &  0 \\
    -1 &  1 & -1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  -2  v_{1}  \\  2  v_{1}  \\ v_{1} \\  -3  v_{1}  \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    \frac{ -2 }{ 3 } c_{2}  & \frac{ 2 }{ 3 } c_{2}  & \frac{ 1 }{ 3 } c_{2}  &  - c_{2}  & c_{1} & c_{1} \\
    \cdot & \frac{ -2 }{ 3 } c_{2}  & \frac{ -1 }{ 3 } c_{2}  & c_{2} &  - c_{1}  &  - c_{1}  \\
    \cdot & \cdot & \frac{ -1 }{ 6 } c_{2}  & \frac{ 1 }{ 2 } c_{2}  & \frac{ -1 }{ 2 } c_{1}  & \frac{ -1 }{ 2 } c_{1}  \\
    \cdot & \cdot & \cdot & \frac{ -3 }{ 2 } c_{2}  & \frac{ 3 }{ 2 } c_{1}  & \frac{ 3 }{ 2 } c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 &  1 & -1 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     1 & -1 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\  - v_{1}  \\ v_{1} \\ v_{2} \\  2  v_{2}  \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} &  - c_{2}  & c_{2} & c_{3} &  2  c_{3}  \\
    \cdot & c_{3} &  - c_{2}  & c_{2} & c_{3} &  2  c_{3}  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  -2  c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{3}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 &  1 &  0 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     1 & -1 &  1 &  1 &  0 &  1 \\
    -1 &  0 &  1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{2} \\  - v_{1}  \\ v_{1} \\  0  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} &  - c_{2}  & c_{2} &  0  & c_{3} \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  0  &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} &  0  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 & -1 &  1 &  0 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     1 & -1 &  0 &  0 &  0 &  1 \\
    -1 &  0 &  1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{2} \\  - v_{1}  \\ v_{1} \\  0  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} &  - c_{2}  & c_{2} &  0  & c_{3} \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  0  &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} &  0  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 &  0 & -1 \\
     1 &  1 &  0 & -1 &  1 &  0 \\
     1 &  0 &  1 &  0 &  0 & -1 \\
     1 &  0 & -1 &  0 &  0 & -1 \\
    -1 &  1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  - v_{1}  \\  0  \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  - c_{2}  &  0  & c_{3} & c_{2} & c_{3} \\
    \cdot & c_{1} &  0  &  - c_{2}  &  - c_{1}  &  - c_{2}  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 &  0 & -1 \\
     1 &  1 &  0 &  1 &  1 & -1 \\
     1 &  0 & -1 &  0 &  0 & -1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v_{2}  \\  - v_{1}  \\  - v_{2}  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{2} & c_{3} &  - c_{2}  &  - c_{3}  &  0  \\
    \cdot & c_{1} & c_{2} &  - c_{1}  &  - c_{2}  &  0  \\
    \cdot & \cdot & c_{3} &  - c_{2}  &  - c_{3}  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     1 &  1 &  0 & -1 &  1 &  0 \\
     1 &  0 &  1 &  0 &  0 & -1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
    -1 &  0 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  - v_{2}  \\ v_{1} \\ v_{1} \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  - c_{2}  & c_{1} & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & c_{3} &  - c_{2}  &  - c_{2}  &  - c_{3}  &  -2  c_{2}  \\
    \cdot & \cdot & c_{1} & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     1 &  1 &  0 & -1 &  1 &  1 \\
     1 &  0 &  1 &  0 & -1 &  0 \\
     1 &  0 & -1 &  1 &  0 & -1 \\
    -1 &  0 & -1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  -3  v_{1}  \\ v_{1} \\ v_{2} \\  2  v_{1}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    \frac{ 1 }{ 2 } c_{1}  & \frac{ -3 }{ 2 } c_{1}  & \frac{ 1 }{ 2 } c_{1}  & c_{2} & c_{1} & c_{2} \\
    \cdot & \frac{ 9 }{ 2 } c_{1}  & \frac{ -3 }{ 2 } c_{1}  &  -3  c_{2}  &  -3  c_{1}  &  -3  c_{2}  \\
    \cdot & \cdot & \frac{ 1 }{ 2 } c_{1}  & c_{2} & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot &  2  c_{1}  &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     1 &  0 &  0 &  0 &  0 & -1 \\
     1 &  0 &  0 &  0 &  0 & -1 \\
    -1 &  0 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  0  \\ v_{2} \\  - v_{1}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  0  & c_{3} &  - c_{2}  & c_{2} & c_{3} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{3} &  - c_{2}  & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     1 &  1 &  0 &  0 &  1 & -1 \\
     1 &  0 &  0 &  0 &  0 & -1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
    -1 &  0 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  - v_{1}  \\ v_{2} \\  0  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  - c_{2}  & c_{3} &  0  & c_{2} & c_{3} \\
    \cdot & c_{1} &  - c_{2}  &  0  &  - c_{1}  &  - c_{2}  \\
    \cdot & \cdot & c_{3} &  0  & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 &  0 &  1 \\
     1 &  1 &  0 & -1 &  1 &  0 \\
     1 &  0 &  1 &  0 &  0 & -1 \\
     1 &  0 & -1 &  0 &  0 &  1 \\
    -1 & -1 &  0 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  - v_{1}  \\ v_{2} \\  0  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{1} &  - c_{2}  &  0  &  - c_{1}  &  - c_{2}  \\
    \cdot & \cdot & c_{3} &  0  & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 & -1 &  1 \\
     1 &  0 & -1 &  0 &  0 &  1 \\
     1 &  1 &  0 &  0 &  1 & -1 \\
     1 &  0 &  0 &  0 &  0 & -1 \\
     1 &  0 & -1 &  0 &  0 &  1 \\
    -1 & -1 &  1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  - v_{1}  \\  2  v_{2}  \\  - v_{2}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  - c_{2}  &  2  c_{3}  &  - c_{3}  & c_{2} & c_{3} \\
    \cdot & c_{1} &  -2  c_{2}  & c_{2} &  - c_{1}  &  - c_{2}  \\
    \cdot & \cdot &  4  c_{3}  &  -2  c_{3}  &  2  c_{2}  &  2  c_{3}  \\
    \cdot & \cdot & \cdot & c_{3} &  - c_{2}  &  - c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 & -1 &  0 \\
     1 &  1 &  0 & -1 & -1 & -1 \\
     1 &  1 &  1 &  0 & -1 & -1 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -1 &  0 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\  0  \\  0  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{3} &  0  &  0  & c_{1} & c_{3} \\
    \cdot & c_{2} &  0  &  0  & c_{3} & c_{2} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 & -1 &  0 \\
     1 &  1 &  0 & -1 & -1 &  0 \\
     1 &  1 &  1 &  0 & -1 &  0 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -1 &  0 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\  - v_{2}  \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{3} &  - c_{3}  & c_{3} & c_{1} & c_{3} \\
    \cdot & c_{2} &  - c_{2}  & c_{2} & c_{3} & c_{2} \\
    \cdot & \cdot & c_{2} &  - c_{2}  &  - c_{3}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{2} & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 & -1 &  0 \\
     1 &  1 &  0 & -1 &  0 & -1 \\
     1 &  1 &  1 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
    -1 &  0 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\  - v_{1}  \\ v_{1} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{2} & c_{3} &  - c_{2}  & c_{2} & c_{2} & c_{3} \\
    \cdot & c_{1} &  - c_{3}  & c_{3} & c_{3} & c_{1} \\
    \cdot & \cdot & c_{2} &  - c_{2}  &  - c_{2}  &  - c_{3}  \\
    \cdot & \cdot & \cdot & c_{2} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{1} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 & -1 &  0 \\
     1 &  1 &  0 &  0 & -1 &  0 \\
     1 &  1 &  0 &  0 & -1 &  0 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -1 &  0 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  0  \\  - v_{1}  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  0  &  - c_{2}  & c_{2} & c_{3} &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 & -1 &  0 \\
     1 &  1 &  0 &  0 & -1 &  1 \\
     1 &  1 &  0 &  0 & -1 &  1 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -1 &  0 & -1 & -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  0  \\  - v_{1}  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  0  &  - c_{2}  & c_{2} & c_{3} &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 & -1 &  0 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
    -1 &  0 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{2} \\  - v_{1}  \\ v_{1} \\  0  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} &  - c_{2}  & c_{2} &  0  & c_{3} \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  0  &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} &  0  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 & -1 &  1 \\
     1 &  1 &  0 & -1 & -1 &  0 \\
     1 &  1 &  1 &  0 & -1 & -1 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -1 & -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  0  \\ v_{2} \\  0  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  0  & c_{3} &  0  & c_{1} & c_{3} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{2} &  0  & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 & -1 &  1 \\
     1 &  1 &  0 & -1 &  1 &  0 \\
     1 &  1 &  1 &  0 & -1 & -1 \\
     0 &  1 & -1 &  1 &  0 &  1 \\
    -1 & -1 &  0 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  3  v_{1}  \\  -2  v_{1}  \\ v_{2} \\  2  v_{1}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    \frac{ 9 }{ 2 } c_{3}  &  -3  c_{3}  & \frac{ -3 }{ 2 } c_{1}  &  3  c_{3}  & \frac{ 3 }{ 2 } c_{3}  & \frac{ -3 }{ 2 } c_{1}  \\
    \cdot &  2  c_{3}  & c_{1} &  -2  c_{3}  &  - c_{3}  & c_{1} \\
    \cdot & \cdot & c_{2} &  - c_{1}  & \frac{ -1 }{ 2 } c_{1}  & c_{2} \\
    \cdot & \cdot & \cdot &  2  c_{3}  & c_{3} &  - c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & \frac{ 1 }{ 2 } c_{3}  & \frac{ -1 }{ 2 } c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 & -1 &  1 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -1 & -1 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  0  \\  - v_{1}  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  0  &  - c_{2}  & c_{2} & c_{3} &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 & -1 &  1 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
    -1 & -1 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{2} \\  - v_{1}  \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} &  - c_{2}  & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 & -1 &  1 \\
     1 &  1 &  0 &  0 &  1 & -1 \\
     1 &  1 &  0 &  0 &  1 & -1 \\
     0 &  1 & -1 & -1 &  0 & -1 \\
    -1 & -1 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v_{2}  \\  2  v_{2}  \\  - v_{1}  \\ v_{1} \\ v_{2} \\  2  v_{2}  \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  -2  c_{3}  & c_{2} &  - c_{2}  &  - c_{3}  &  -2  c_{3}  \\
    \cdot &  4  c_{3}  &  -2  c_{2}  &  2  c_{2}  &  2  c_{3}  &  4  c_{3}  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  -2  c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{3}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  0 & -1 \\
     1 &  1 &  0 & -1 &  0 & -1 \\
     1 &  1 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\  - v_{2}  \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} &  - c_{3}  & c_{3} & c_{2} & c_{3} \\
    \cdot & c_{3} &  - c_{3}  & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & c_{3} &  - c_{3}  &  - c_{2}  &  - c_{3}  \\
    \cdot & \cdot & \cdot & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  0 & -1 \\
     1 &  1 &  0 & -1 &  0 &  0 \\
     1 &  1 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{2}  \\  0  \\  - v_{2}  \\  2  v_{2}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     4  c_{3}  &  0  &  -2  c_{3}  &  4  c_{3}  &  2  c_{2}  &  2  c_{3}  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{3} &  -2  c_{3}  &  - c_{2}  &  - c_{3}  \\
    \cdot & \cdot & \cdot &  4  c_{3}  &  2  c_{2}  &  2  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  0 & -1 \\
     1 &  1 &  0 & -1 &  0 &  1 \\
     1 &  1 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 & -1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  3  v_{2}  \\  - v_{2}  \\  - v_{2}  \\  3  v_{2}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     9  c_{3}  &  -3  c_{3}  &  -3  c_{3}  &  9  c_{3}  &  3  c_{2}  &  3  c_{3}  \\
    \cdot & c_{3} & c_{3} &  -3  c_{3}  &  - c_{2}  &  - c_{3}  \\
    \cdot & \cdot & c_{3} &  -3  c_{3}  &  - c_{2}  &  - c_{3}  \\
    \cdot & \cdot & \cdot &  9  c_{3}  &  3  c_{2}  &  3  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  0 & -1 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  - v_{1}  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  0 &  0 \\
     1 &  1 &  0 & -1 &  0 & -1 \\
     1 &  1 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{2} \\  0  \\  0  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} &  0  &  0  & c_{2} & c_{3} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  0 &  0 \\
     1 &  1 &  0 & -1 &  0 &  0 \\
     1 &  1 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  0  \\  0  \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  0  &  0  & c_{3} & c_{2} & c_{3} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  0 &  1 \\
     1 &  1 &  0 & -1 & -1 &  0 \\
     1 &  1 &  1 &  0 &  0 & -1 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
    -1 & -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v_{1}  \\ v_{1} \\ v_{2} \\  - v_{1}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     - c_{1}  & c_{1} & c_{3} &  - c_{1}  & c_{1} & c_{3} \\
    \cdot &  - c_{1}  &  - c_{3}  & c_{1} &  - c_{1}  &  - c_{3}  \\
    \cdot & \cdot & c_{2} & c_{3} &  - c_{3}  & c_{2} \\
    \cdot & \cdot & \cdot &  - c_{1}  & c_{1} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot &  - c_{1}  &  - c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  0 &  1 \\
     1 &  1 &  0 & -1 &  0 & -1 \\
     1 &  1 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 & -1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v_{2}  \\ v_{2} \\ v_{2} \\  - v_{2}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  - c_{3}  &  - c_{3}  & c_{3} &  - c_{2}  &  - c_{3}  \\
    \cdot & c_{3} & c_{3} &  - c_{3}  & c_{2} & c_{3} \\
    \cdot & \cdot & c_{3} &  - c_{3}  & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & c_{3} &  - c_{2}  &  - c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  0 &  1 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 & -1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  - v_{1}  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  1 & -1 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     0 & -1 &  1 &  1 &  0 &  1 \\
    -1 &  1 &  1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  2  v_{2}  \\  - v_{1}  \\ v_{1} \\ v_{2} \\  2  v_{2}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  2  c_{1}  & c_{2} &  - c_{2}  & c_{1} &  2  c_{1}  \\
    \cdot &  4  c_{1}  &  2  c_{2}  &  -2  c_{2}  &  2  c_{1}  &  4  c_{1}  \\
    \cdot & \cdot & c_{3} &  - c_{3}  & c_{2} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & c_{3} &  - c_{2}  &  -2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} &  2  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  1 & -1 \\
     1 &  1 &  0 &  0 & -1 &  0 \\
     1 &  1 &  0 &  0 & -1 &  0 \\
     0 & -1 &  1 &  1 &  0 &  1 \\
    -1 &  1 &  0 &  0 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{2} \\  - v_{1}  \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} &  - c_{2}  & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  1 & -1 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     0 & -1 &  0 &  0 &  0 &  1 \\
    -1 &  1 &  1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{2} \\  - v_{1}  \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} &  - c_{2}  & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  1 & -1 \\
     1 &  1 &  0 &  0 &  1 & -1 \\
     1 &  1 &  0 &  0 &  1 & -1 \\
     0 & -1 & -1 & -1 &  0 &  1 \\
    -1 &  1 &  1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v_{2}  \\  0  \\  - v_{1}  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  0  & c_{2} &  - c_{2}  &  - c_{3}  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  1 &  0 \\
     1 &  1 &  0 & -1 & -1 & -1 \\
     1 &  1 &  1 &  0 & -1 & -1 \\
     0 & -1 &  1 &  1 &  0 &  1 \\
    -1 &  0 &  1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v_{1}  \\ v_{2} \\  2  v_{1}  \\  -2  v_{1}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    \frac{ -1 }{ 2 } c_{3}  & \frac{ -1 }{ 2 } c_{2}  & c_{3} &  - c_{3}  & \frac{ 1 }{ 2 } c_{3}  & \frac{ -1 }{ 2 } c_{2}  \\
    \cdot & c_{1} & c_{2} &  - c_{2}  & \frac{ 1 }{ 2 } c_{2}  & c_{1} \\
    \cdot & \cdot &  -2  c_{3}  &  2  c_{3}  &  - c_{3}  & c_{2} \\
    \cdot & \cdot & \cdot &  -2  c_{3}  & c_{3} &  - c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \frac{ -1 }{ 2 } c_{3}  & \frac{ 1 }{ 2 } c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{1} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  1 &  0 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     0 & -1 &  1 &  1 &  0 &  1 \\
    -1 &  0 &  1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{2} \\  - v_{1}  \\ v_{1} \\  0  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} &  - c_{2}  & c_{2} &  0  & c_{3} \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  0  &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} &  0  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  1 &  0 \\
     1 &  1 &  0 &  0 & -1 &  1 \\
     1 &  1 &  0 &  0 &  1 & -1 \\
     0 & -1 &  1 & -1 &  0 & -1 \\
    -1 &  0 & -1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  - v_{1}  \\ v_{2} \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     - c_{1}  & c_{1} & c_{2} &  - c_{1}  & c_{2} & c_{2} \\
    \cdot &  - c_{1}  &  - c_{2}  & c_{1} &  - c_{2}  &  - c_{2}  \\
    \cdot & \cdot & c_{3} & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot &  - c_{1}  & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  1 &  0 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     0 & -1 &  0 &  0 &  0 &  1 \\
    -1 &  0 &  1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{2} \\  - v_{1}  \\ v_{1} \\  0  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} &  - c_{2}  & c_{2} &  0  & c_{3} \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  0  &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} &  0  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  1 &  1 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     0 & -1 &  1 &  1 &  0 &  1 \\
    -1 & -1 &  1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  -2  v_{2}  \\  - v_{1}  \\ v_{1} \\ v_{2} \\  -2  v_{2}  \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  -2  c_{3}  &  - c_{2}  & c_{2} & c_{3} &  -2  c_{3}  \\
    \cdot &  4  c_{3}  &  2  c_{2}  &  -2  c_{2}  &  -2  c_{3}  &  4  c_{3}  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  2  c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  -2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  -2  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{3}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 & -1 &  1 &  1 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     0 & -1 &  0 &  0 &  0 &  1 \\
    -1 & -1 &  1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{2} \\  - v_{1}  \\ v_{1} \\  - v_{2}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} &  - c_{2}  & c_{2} &  - c_{3}  & c_{3} \\
    \cdot & \cdot & c_{1} &  - c_{1}  & c_{2} &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} &  - c_{2}  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  - c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 & -1 & -1 \\
     1 &  1 &  0 & -1 & -1 &  0 \\
     1 &  0 &  1 &  0 & -1 &  1 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -1 &  1 &  0 & -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\  - v_{2}  \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{3} &  - c_{3}  & c_{3} & c_{1} & c_{3} \\
    \cdot & c_{2} &  - c_{2}  & c_{2} & c_{3} & c_{2} \\
    \cdot & \cdot & c_{2} &  - c_{2}  &  - c_{3}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{2} & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 & -1 & -1 \\
     1 &  1 &  0 & -1 & -1 &  0 \\
     1 &  0 &  1 &  0 &  1 & -1 \\
     0 &  1 &  1 & -1 &  0 &  1 \\
    -1 &  1 &  0 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{1} \\  - v_{1}  \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{2} & c_{3} &  - c_{3}  & c_{2} & c_{3} & c_{2} \\
    \cdot &  - c_{1}  & c_{1} & c_{3} &  - c_{1}  & c_{3} \\
    \cdot & \cdot &  - c_{1}  &  - c_{3}  & c_{1} &  - c_{3}  \\
    \cdot & \cdot & \cdot & c_{2} & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot &  - c_{1}  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 & -1 & -1 \\
     1 &  1 &  0 &  0 & -1 &  0 \\
     1 &  0 &  0 &  0 & -1 &  0 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -1 &  1 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  0  \\  - v_{2}  \\  2  v_{2}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  0  &  - c_{2}  &  2  c_{2}  & c_{1} & c_{2} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \frac{ 1 }{ 2 } c_{3}  &  - c_{3}  &  - c_{2}  & \frac{ -1 }{ 2 } c_{3}  \\
    \cdot & \cdot & \cdot &  2  c_{3}  &  2  c_{2}  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & \frac{ 1 }{ 2 } c_{3}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 & -1 & -1 \\
     1 &  1 &  0 &  0 & -1 &  1 \\
     1 &  0 &  0 &  0 & -1 &  0 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -1 &  1 & -1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  - v_{2}  \\  - v_{2}  \\  3  v_{2}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  - c_{3}  &  - c_{3}  &  3  c_{3}  & c_{1} & c_{3} \\
    \cdot &  - c_{2}  &  - c_{2}  &  3  c_{2}  &  - c_{3}  & c_{2} \\
    \cdot & \cdot &  - c_{2}  &  3  c_{2}  &  - c_{3}  & c_{2} \\
    \cdot & \cdot & \cdot &  -9  c_{2}  &  3  c_{3}  &  -3  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  - c_{2}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 & -1 & -1 \\
     1 &  1 &  0 &  1 &  0 & -1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
    -1 &  1 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v_{1}  \\ v_{2} \\  - v_{1}  \\ v_{1} \\  - v_{2}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  - c_{3}  & c_{1} &  - c_{1}  & c_{3} &  - c_{3}  \\
    \cdot & c_{2} &  - c_{3}  & c_{3} &  - c_{2}  & c_{2} \\
    \cdot & \cdot & c_{1} &  - c_{1}  & c_{3} &  - c_{3}  \\
    \cdot & \cdot & \cdot & c_{1} &  - c_{3}  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{2} &  - c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 & -1 &  0 \\
     1 &  1 &  0 & -1 & -1 & -1 \\
     1 &  0 &  1 &  0 & -1 &  0 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -1 &  0 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\  0  \\  0  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{3} &  0  &  0  & c_{1} & c_{3} \\
    \cdot & c_{2} &  0  &  0  & c_{3} & c_{2} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 & -1 &  0 \\
     1 &  1 &  0 & -1 & -1 &  0 \\
     1 &  0 &  1 &  0 & -1 &  0 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -1 &  0 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{1} \\  0  \\ v_{1} \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{2} &  0  & c_{2} & c_{1} &  2  c_{2}  \\
    \cdot & \frac{ 1 }{ 2 } c_{3}  &  0  & \frac{ 1 }{ 2 } c_{3}  & c_{2} & c_{3} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \frac{ 1 }{ 2 } c_{3}  & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  2  c_{3}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 & -1 &  0 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     1 &  0 &  0 &  0 & -1 &  0 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -1 &  0 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\  0  \\  0  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{3} &  0  &  0  & c_{1} & c_{3} \\
    \cdot & c_{2} &  0  &  0  & c_{3} & c_{2} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 & -1 &  0 \\
     1 &  1 &  0 &  0 & -1 &  0 \\
     1 &  0 &  0 &  0 & -1 &  0 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -1 &  0 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  0  \\  0  \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  0  &  0  & c_{3} & c_{1} & c_{3} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{2} & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 & -1 &  0 \\
     1 &  1 &  0 &  1 & -1 & -1 \\
     1 &  0 & -1 &  0 &  1 &  0 \\
     0 &  1 &  1 & -1 &  0 &  1 \\
    -1 &  0 &  1 &  0 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  - v_{1}  \\ v_{1} \\ v_{2} \\  0  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  - c_{1}  & c_{1} & c_{2} &  0  & c_{2} \\
    \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  0  &  - c_{2}  \\
    \cdot & \cdot & c_{1} & c_{2} &  0  & c_{2} \\
    \cdot & \cdot & \cdot & c_{3} &  0  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 & -1 &  0 \\
     1 &  1 &  0 &  1 &  0 & -1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
    -1 &  0 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v_{1}  \\ v_{2} \\  - v_{1}  \\ v_{1} \\  0  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  - c_{3}  & c_{1} &  - c_{1}  &  0  &  - c_{3}  \\
    \cdot & c_{2} &  - c_{3}  & c_{3} &  0  & c_{2} \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  0  &  - c_{3}  \\
    \cdot & \cdot & \cdot & c_{1} &  0  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 & -1 &  1 \\
     1 &  1 &  0 & -1 & -1 & -1 \\
     1 &  0 &  1 &  0 & -1 & -1 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -1 & -1 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  - v_{1}  \\  -2  v_{1}  \\ v_{1} \\ v_{2} \\  -2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & \frac{ 1 }{ 2 } c_{3}  & c_{3} & \frac{ -1 }{ 2 } c_{3}  & c_{1} & c_{3} \\
    \cdot & \frac{ 1 }{ 2 } c_{2}  & c_{2} & \frac{ -1 }{ 2 } c_{2}  & \frac{ 1 }{ 2 } c_{3}  & c_{2} \\
    \cdot & \cdot &  2  c_{2}  &  - c_{2}  & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \frac{ 1 }{ 2 } c_{2}  & \frac{ -1 }{ 2 } c_{3}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  2  c_{2}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 & -1 &  1 \\
     1 &  1 &  0 & -1 & -1 &  0 \\
     1 &  0 &  1 &  0 & -1 & -1 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -1 & -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  0  \\ v_{2} \\  0  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  0  & c_{3} &  0  & c_{1} & c_{3} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{2} &  0  & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 & -1 &  1 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     1 &  0 &  0 &  0 & -1 &  0 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -1 & -1 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\ v_{2} \\  - v_{2}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{3} & c_{3} &  - c_{3}  & c_{1} & c_{3} \\
    \cdot &  - c_{2}  &  - c_{2}  & c_{2} & c_{3} &  - c_{2}  \\
    \cdot & \cdot &  - c_{2}  & c_{2} & c_{3} &  - c_{2}  \\
    \cdot & \cdot & \cdot &  - c_{2}  &  - c_{3}  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  - c_{2}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 & -1 &  1 \\
     1 &  1 &  0 &  1 &  0 & -1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
    -1 & -1 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v_{1}  \\ v_{2} \\  - v_{1}  \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  - c_{3}  & c_{1} &  - c_{1}  &  - c_{3}  &  - c_{3}  \\
    \cdot & c_{2} &  - c_{3}  & c_{3} & c_{2} & c_{2} \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{3}  &  - c_{3}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 & -1 \\
     1 &  1 &  0 & -1 &  0 & -1 \\
     1 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{1}  \\ v_{1} \\  0  \\ v_{1} \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     4  c_{1}  &  2  c_{1}  &  0  &  2  c_{1}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & c_{1} &  0  & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 & -1 \\
     1 &  1 &  0 & -1 &  0 &  0 \\
     1 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  0  \\  0  \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  0  &  0  & c_{3} & c_{2} & c_{3} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 & -1 \\
     1 &  1 &  0 & -1 &  0 &  1 \\
     1 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 & -1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ \frac{ -1 }{ 2 } v_{2}  \\  0  \\ \frac{ 3 }{ 2 } v_{2}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     -2  c_{1}  & c_{1} &  0  &  -3  c_{1}  & c_{3} &  -2  c_{1}  \\
    \cdot & \frac{ -1 }{ 2 } c_{1}  &  0  & \frac{ 3 }{ 2 } c_{1}  & \frac{ -1 }{ 2 } c_{3}  & c_{1} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \frac{ -9 }{ 2 } c_{1}  & \frac{ 3 }{ 2 } c_{3}  &  -3  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  -2  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 & -1 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     1 &  0 &  0 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  0  \\  0  \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  0  &  0  & c_{3} & c_{2} & c_{3} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 & -1 \\
     1 &  1 &  0 &  1 & -1 &  0 \\
     1 &  0 & -1 &  0 &  0 & -1 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
    -1 &  1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{2}  \\  - v_{1}  \\ v_{2} \\ v_{1} \\  2  v_{2}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     4  c_{3}  &  -2  c_{2}  &  2  c_{3}  &  2  c_{2}  &  4  c_{3}  &  2  c_{3}  \\
    \cdot & c_{1} &  - c_{2}  &  - c_{1}  &  -2  c_{2}  &  - c_{2}  \\
    \cdot & \cdot & c_{3} & c_{2} &  2  c_{3}  & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} &  2  c_{2}  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot &  4  c_{3}  &  2  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 & -1 \\
     1 &  1 &  0 &  1 &  0 & -1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v_{1}  \\  0  \\  - v_{1}  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  0  & c_{1} &  - c_{1}  &  - c_{2}  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 & -1 \\
     1 &  1 &  0 &  1 &  0 & -1 \\
     1 &  0 & -1 &  0 &  0 &  1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 & -1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  -2  v_{1}  \\ v_{1} \\  -2  v_{1}  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
     4  c_{1}  &  -2  c_{1}  &  4  c_{1}  &  -2  c_{1}  &  -2  c_{2}  &  0  \\
    \cdot & c_{1} &  -2  c_{1}  & c_{1} & c_{2} &  0  \\
    \cdot & \cdot &  4  c_{1}  &  -2  c_{1}  &  -2  c_{2}  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     1 &  1 &  0 & -1 &  0 & -1 \\
     1 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{1} \\ v_{1} \\  0  \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{1} & c_{1} &  0  & c_{2} &  2  c_{1}  \\
    \cdot & c_{1} & c_{1} &  0  & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & c_{1} &  0  & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     1 &  1 &  0 & -1 &  0 &  0 \\
     1 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  0  \\ v_{1} \\ v_{1} \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  0  & c_{1} & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{1} & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     1 &  1 &  0 & -1 &  0 &  1 \\
     1 &  0 &  1 &  0 & -1 &  0 \\
     0 &  0 &  0 &  1 &  0 & -1 \\
    -1 &  0 & -1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  - v_{1}  \\ v_{1} \\ v_{2} \\  2  v_{1}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    \frac{ 1 }{ 2 } c_{2}  & \frac{ -1 }{ 2 } c_{2}  & \frac{ 1 }{ 2 } c_{2}  &  - c_{1}  & c_{2} &  - c_{1}  \\
    \cdot & \frac{ 1 }{ 2 } c_{2}  & \frac{ -1 }{ 2 } c_{2}  & c_{1} &  - c_{2}  & c_{1} \\
    \cdot & \cdot & \frac{ 1 }{ 2 } c_{2}  &  - c_{1}  & c_{2} &  - c_{1}  \\
    \cdot & \cdot & \cdot & c_{3} &  -2  c_{1}  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot &  2  c_{2}  &  -2  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     1 &  1 &  0 & -1 &  0 &  1 \\
     1 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 & -1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  - v_{1}  \\ v_{1} \\  2  v_{1}  \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  - c_{1}  & c_{1} &  2  c_{1}  & c_{2} &  2  c_{1}  \\
    \cdot & c_{1} &  - c_{1}  &  -2  c_{1}  &  - c_{2}  &  -2  c_{1}  \\
    \cdot & \cdot & c_{1} &  2  c_{1}  & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & \cdot &  4  c_{1}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     1 &  0 &  0 &  0 &  0 & -1 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
    -1 &  0 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{1} \\ v_{2} \\  - v_{1}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{3} & c_{1} &  - c_{3}  & c_{3} & c_{1} \\
    \cdot &  - c_{2}  & c_{3} & c_{2} &  - c_{2}  & c_{3} \\
    \cdot & \cdot & c_{1} &  - c_{3}  & c_{3} & c_{1} \\
    \cdot & \cdot & \cdot &  - c_{2}  & c_{2} &  - c_{3}  \\
    \cdot & \cdot & \cdot & \cdot &  - c_{2}  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{1} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     1 &  0 &  0 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  0  \\ v_{2} \\  0  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  0  & c_{3} &  0  & c_{2} & c_{3} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{3} &  0  & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     1 &  1 &  0 &  0 &  1 & -1 \\
     1 &  0 &  0 &  0 &  0 & -1 \\
     0 &  0 & -1 &  0 &  0 &  1 \\
    -1 &  0 &  1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  - v_{1}  \\ v_{2} \\ v_{1} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  - c_{3}  & c_{1} & c_{3} & c_{3} & c_{1} \\
    \cdot & c_{2} &  - c_{3}  &  - c_{2}  &  - c_{2}  &  - c_{3}  \\
    \cdot & \cdot & c_{1} & c_{3} & c_{3} & c_{1} \\
    \cdot & \cdot & \cdot & c_{2} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{1} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     1 &  1 &  0 &  1 & -1 & -1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
    -1 &  0 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  - v_{1}  \\ v_{2} \\ v_{1} \\  0  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  - c_{2}  & c_{3} & c_{2} &  0  & c_{3} \\
    \cdot & c_{1} &  - c_{2}  &  - c_{1}  &  0  &  - c_{2}  \\
    \cdot & \cdot & c_{3} & c_{2} &  0  & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} &  0  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     1 &  1 &  0 &  1 & -1 &  0 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
    -1 &  0 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  - v_{1}  \\ v_{2} \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  - c_{2}  & c_{3} & c_{2} & c_{3} & c_{3} \\
    \cdot & c_{1} &  - c_{2}  &  - c_{1}  &  - c_{2}  &  - c_{2}  \\
    \cdot & \cdot & c_{3} & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 &  1 \\
     1 &  1 &  0 & -1 & -1 &  0 \\
     1 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
    -1 & -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  - v_{1}  \\ v_{2} \\ v_{1} \\  -2  v_{1}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \frac{ -1 }{ 2 } c_{2}  &  - c_{3}  & \frac{ 1 }{ 2 } c_{2}  &  - c_{2}  &  - c_{3}  \\
    \cdot & \cdot & c_{1} & c_{3} &  -2  c_{3}  & c_{1} \\
    \cdot & \cdot & \cdot & \frac{ -1 }{ 2 } c_{2}  & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot &  -2  c_{2}  &  -2  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{1} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 &  1 \\
     1 &  1 &  0 & -1 &  0 & -1 \\
     1 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 & -1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  - v_{1}  \\  -2  v_{1}  \\ v_{1} \\ v_{2} \\  -2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{1} &  2  c_{1}  &  - c_{1}  &  - c_{2}  &  2  c_{1}  \\
    \cdot & \cdot &  4  c_{1}  &  -2  c_{1}  &  -2  c_{2}  &  4  c_{1}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  -2  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  -2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 &  1 \\
     1 &  1 &  0 & -1 &  0 &  0 \\
     1 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 & -1 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\ v_{2} \\  0  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{3} &  0  & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 &  1 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     1 &  0 &  0 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 & -1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  0  \\  2  v_{2}  \\  - v_{2}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  0  &  2  c_{3}  &  - c_{3}  & c_{2} & c_{3} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  4  c_{3}  &  -2  c_{3}  &  2  c_{2}  &  2  c_{3}  \\
    \cdot & \cdot & \cdot & c_{3} &  - c_{2}  &  - c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 &  1 \\
     1 &  1 &  0 &  1 & -1 & -1 \\
     1 &  0 & -1 &  0 &  0 &  1 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
    -1 & -1 &  1 & -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  - v_{1}  \\ v_{2} \\ v_{1} \\  - v_{2}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{1} &  - c_{2}  &  - c_{1}  & c_{2} &  - c_{2}  \\
    \cdot & \cdot & c_{3} & c_{2} &  - c_{3}  & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} &  - c_{2}  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  - c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  1 & -1 \\
     1 &  1 &  0 &  1 & -1 &  0 \\
     1 &  0 & -1 &  0 &  1 & -1 \\
     0 & -1 &  1 & -1 &  0 & -1 \\
    -1 &  1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  - v_{1}  \\ v_{2} \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  - c_{2}  & c_{3} & c_{2} & c_{3} & c_{3} \\
    \cdot & c_{1} &  - c_{2}  &  - c_{1}  &  - c_{2}  &  - c_{2}  \\
    \cdot & \cdot & c_{3} & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  1 &  0 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     1 &  0 &  0 &  0 & -1 &  0 \\
     0 & -1 &  1 &  1 &  0 &  1 \\
    -1 &  0 &  1 &  0 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\  2  v_{1}  \\  -2  v_{1}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    \frac{ 1 }{ 2 } c_{2}  & \frac{ 1 }{ 2 } c_{3}  & c_{2} &  - c_{2}  & \frac{ 1 }{ 2 } c_{2}  & \frac{ 1 }{ 2 } c_{3}  \\
    \cdot & c_{1} & c_{3} &  - c_{3}  & \frac{ 1 }{ 2 } c_{3}  & c_{1} \\
    \cdot & \cdot &  2  c_{2}  &  -2  c_{2}  & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot &  2  c_{2}  &  - c_{2}  &  - c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \frac{ 1 }{ 2 } c_{2}  & \frac{ 1 }{ 2 } c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{1} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  1 &  0 \\
     1 &  1 &  0 &  1 & -1 & -1 \\
     1 &  0 & -1 &  0 &  1 &  0 \\
     0 & -1 &  1 & -1 &  0 & -1 \\
    -1 &  0 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  - v_{1}  \\ v_{2} \\ v_{1} \\  0  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  - c_{2}  & c_{3} & c_{2} &  0  & c_{3} \\
    \cdot & c_{1} &  - c_{2}  &  - c_{1}  &  0  &  - c_{2}  \\
    \cdot & \cdot & c_{3} & c_{2} &  0  & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} &  0  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  0 &  1 &  1 \\
     1 &  1 &  0 & -1 & -1 &  0 \\
     1 &  0 &  1 &  0 &  1 & -1 \\
     0 & -1 &  1 & -1 &  0 & -1 \\
    -1 & -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v_{1}  \\ v_{1} \\ v_{2} \\  - v_{1}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     - c_{2}  & c_{2} &  - c_{3}  &  - c_{2}  & c_{2} &  - c_{3}  \\
    \cdot &  - c_{2}  & c_{3} & c_{2} &  - c_{2}  & c_{3} \\
    \cdot & \cdot & c_{1} &  - c_{3}  & c_{3} & c_{1} \\
    \cdot & \cdot & \cdot &  - c_{2}  & c_{2} &  - c_{3}  \\
    \cdot & \cdot & \cdot & \cdot &  - c_{2}  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{1} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  1 & -1 & -1 \\
     1 &  1 &  0 & -1 & -1 &  0 \\
     1 & -1 &  1 &  0 & -1 &  1 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -1 &  1 &  0 & -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{1} \\ \frac{ -1 }{ 2 } v_{1}  \\ v_{1} \\ v_{2} \\ \frac{ 3 }{ 2 } v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & \frac{ 2 }{ 3 } c_{3}  & \frac{ -1 }{ 3 } c_{3}  & \frac{ 2 }{ 3 } c_{3}  & c_{1} & c_{3} \\
    \cdot & \frac{ 2 }{ 3 } c_{2}  & \frac{ -1 }{ 3 } c_{2}  & \frac{ 2 }{ 3 } c_{2}  & \frac{ 2 }{ 3 } c_{3}  & c_{2} \\
    \cdot & \cdot & \frac{ 1 }{ 6 } c_{2}  & \frac{ -1 }{ 3 } c_{2}  & \frac{ -1 }{ 3 } c_{3}  & \frac{ -1 }{ 2 } c_{2}  \\
    \cdot & \cdot & \cdot & \frac{ 2 }{ 3 } c_{2}  & \frac{ 2 }{ 3 } c_{3}  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & \frac{ 3 }{ 2 } c_{2}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  1 & -1 & -1 \\
     1 &  1 &  0 & -1 & -1 &  1 \\
     1 & -1 &  1 &  0 & -1 &  0 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -1 &  1 & -1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  0  \\  0  \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  0  &  0  & c_{3} & c_{1} & c_{3} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{2} & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  1 & -1 &  0 \\
     1 &  1 &  0 & -1 &  0 & -1 \\
     1 & -1 &  1 &  0 &  0 &  1 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
    -1 &  0 &  1 & -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\  - v_{1}  \\ v_{1} \\  3  v_{1}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     - c_{3}  & c_{1} & c_{3} &  - c_{3}  &  -3  c_{3}  & c_{1} \\
    \cdot & c_{2} &  - c_{1}  & c_{1} &  3  c_{1}  & c_{2} \\
    \cdot & \cdot &  - c_{3}  & c_{3} &  3  c_{3}  &  - c_{1}  \\
    \cdot & \cdot & \cdot &  - c_{3}  &  -3  c_{3}  & c_{1} \\
    \cdot & \cdot & \cdot & \cdot &  -9  c_{3}  &  3  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  1 &  0 & -1 \\
     1 &  1 &  0 & -1 &  0 & -1 \\
     1 & -1 &  1 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{1} \\  0  \\ \frac{ 1 }{ 2 } v_{1}  \\ v_{2} \\ \frac{ 3 }{ 2 } v_{1}  \end{bmatrix}
  \begin{bmatrix}
     4  c_{2}  &  4  c_{2}  &  0  &  2  c_{2}  & c_{1} &  6  c_{2}  \\
    \cdot &  4  c_{2}  &  0  &  2  c_{2}  & c_{1} &  6  c_{2}  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{2} & \frac{ 1 }{ 2 } c_{1}  &  3  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & \frac{ 3 }{ 2 } c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  9  c_{2}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  1 &  0 & -1 \\
     1 &  1 &  0 & -1 &  0 & -1 \\
     1 & -1 &  1 &  0 &  0 &  1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 & -1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  3  v_{1}  \\  - v_{1}  \\ v_{1} \\ v_{2} \\  3  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  3  c_{1}  &  - c_{1}  & c_{1} & c_{2} &  3  c_{1}  \\
    \cdot &  9  c_{1}  &  -3  c_{1}  &  3  c_{1}  &  3  c_{2}  &  9  c_{1}  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  -3  c_{1}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  3  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  3  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  9  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  1 &  0 & -1 \\
     1 &  1 &  0 & -1 &  0 &  0 \\
     1 & -1 &  1 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  0 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{1} \\  0  \\  2  v_{1}  \\ v_{2} \\  3  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{1} &  0  &  2  c_{1}  & c_{2} &  3  c_{1}  \\
    \cdot & c_{1} &  0  &  2  c_{1}  & c_{2} &  3  c_{1}  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot &  4  c_{1}  &  2  c_{2}  &  6  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  3  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  9  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 & -1 &  1 &  0 & -1 \\
     1 &  1 &  0 & -1 &  0 &  1 \\
     1 & -1 &  1 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 & -1 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  0  \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 &  0 &  0 & -1 & -1 \\
     1 &  0 &  0 &  0 & -1 & -1 \\
     1 &  0 &  0 &  0 & -1 &  1 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -1 &  1 &  1 & -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  - v_{1}  \\ v_{1} \\  0  \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  - c_{2}  & c_{2} &  0  & c_{3} &  0  \\
    \cdot & c_{1} &  - c_{1}  &  0  &  - c_{2}  &  0  \\
    \cdot & \cdot & c_{1} &  0  & c_{2} &  0  \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 &  0 &  0 & -1 & -1 \\
     1 &  0 &  0 &  0 & -1 &  0 \\
     1 &  0 &  0 &  0 & -1 &  0 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -1 &  1 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  0  \\  - v_{1}  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  0  &  - c_{2}  & c_{2} & c_{3} &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 &  0 &  0 & -1 & -1 \\
     1 &  0 &  0 &  0 & -1 &  0 \\
     1 &  0 &  0 &  0 & -1 &  1 \\
     0 &  1 &  1 &  1 &  0 & -1 \\
    -1 &  1 &  0 & -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{1} \\  -2  v_{1}  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{3} &  -2  c_{3}  & c_{3} & c_{1} &  0  \\
    \cdot & \frac{ -1 }{ 2 } c_{2}  & c_{2} & \frac{ -1 }{ 2 } c_{2}  & c_{3} &  0  \\
    \cdot & \cdot &  -2  c_{2}  & c_{2} &  -2  c_{3}  &  0  \\
    \cdot & \cdot & \cdot & \frac{ -1 }{ 2 } c_{2}  & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 &  0 &  0 & -1 &  0 \\
     1 &  0 &  0 &  0 & -1 &  0 \\
     1 &  0 &  0 &  0 &  1 & -1 \\
     0 &  1 &  1 & -1 &  0 &  1 \\
    -1 &  0 &  0 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  - v_{1}  \\ v_{1} \\  2  v_{2}  \\ v_{2} \\  2  v_{2}  \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  - c_{2}  & c_{2} &  2  c_{3}  & c_{3} &  2  c_{3}  \\
    \cdot & c_{1} &  - c_{1}  &  -2  c_{2}  &  - c_{2}  &  -2  c_{2}  \\
    \cdot & \cdot & c_{1} &  2  c_{2}  & c_{2} &  2  c_{2}  \\
    \cdot & \cdot & \cdot &  4  c_{3}  &  2  c_{3}  &  4  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{3}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 &  0 &  0 & -1 &  0 \\
     1 &  0 &  0 &  0 &  0 & -1 \\
     1 &  0 &  0 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
    -1 &  0 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\  - v_{1}  \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} &  - c_{2}  & c_{2} & c_{3} & c_{3} \\
    \cdot & c_{3} &  - c_{2}  & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 &  0 &  0 & -1 &  1 \\
     1 &  0 &  0 &  0 &  0 & -1 \\
     1 &  0 &  0 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
    -1 & -1 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\  - v_{1}  \\ v_{1} \\  2  v_{2}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} &  - c_{2}  & c_{2} &  2  c_{3}  & c_{3} \\
    \cdot & c_{3} &  - c_{2}  & c_{2} &  2  c_{3}  & c_{3} \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  -2  c_{2}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} &  2  c_{2}  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot &  4  c_{3}  &  2  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  0 &  1 \\
     1 &  0 &  0 &  0 &  0 & -1 \\
     1 &  0 &  0 &  0 &  0 & -1 \\
     1 &  0 &  0 &  0 &  1 & -1 \\
     0 &  0 &  0 & -1 &  0 &  1 \\
    -1 &  1 &  1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  - v_{1}  \\ v_{1} \\ v_{2} \\  0  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  - c_{2}  & c_{2} & c_{3} &  0  & c_{3} \\
    \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  0  &  - c_{2}  \\
    \cdot & \cdot & c_{1} & c_{2} &  0  & c_{2} \\
    \cdot & \cdot & \cdot & c_{3} &  0  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 &  1 \\
     1 &  0 & -1 & -1 &  0 &  0 \\
     1 &  1 &  0 & -1 & -1 &  0 \\
     1 &  1 &  1 &  0 & -1 & -1 \\
    -1 &  0 &  1 &  1 &  0 &  0 \\
    -1 &  0 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{1} \\  0  \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{3} &  0  & c_{1} & c_{3} & c_{1} \\
    \cdot & c_{2} &  0  & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{3} & c_{1} \\
    \cdot & \cdot & \cdot & \cdot & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{1} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 &  1 \\
     1 &  0 & -1 & -1 &  0 &  1 \\
     1 &  1 &  0 & -1 & -1 &  0 \\
     1 &  1 &  1 &  0 & -1 & -1 \\
    -1 &  0 &  1 &  1 &  0 & -1 \\
    -1 & -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{1} \\ v_{2} \\  0  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{1} & c_{3} &  0  & c_{1} & c_{3} \\
    \cdot & \cdot & c_{2} &  0  & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 &  1 \\
     1 &  0 & -1 & -1 &  0 &  1 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
    -1 &  0 &  1 &  1 &  0 & -1 \\
    -1 & -1 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{2} \\  - v_{1}  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} &  - c_{2}  & c_{2} & c_{3} &  0  \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 &  1 \\
     1 &  0 & -1 & -1 &  1 &  1 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
    -1 & -1 &  1 &  1 &  0 &  0 \\
    -1 & -1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  - v_{1}  \\ v_{1} \\  - v_{2}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{1} &  - c_{1}  & c_{2} &  - c_{2}  \\
    \cdot & \cdot & \cdot & c_{1} &  - c_{2}  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  - c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 &  1 \\
     1 &  0 & -1 &  0 & -1 &  0 \\
     1 &  1 &  0 & -1 &  0 & -1 \\
     1 &  0 &  1 &  0 & -1 &  0 \\
    -1 &  1 &  0 &  1 &  0 & -1 \\
    -1 &  0 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\  0  \\ v_{1} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{2} &  0  & c_{1} & c_{1} & c_{2} \\
    \cdot & c_{3} &  0  & c_{2} & c_{2} & c_{3} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 &  1 \\
     1 &  0 & -1 &  0 & -1 &  0 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     1 &  0 &  0 &  0 & -1 &  0 \\
    -1 &  1 &  1 &  1 &  0 & -1 \\
    -1 &  0 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\  0  \\ v_{1} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{3} &  0  & c_{1} & c_{1} & c_{3} \\
    \cdot & c_{2} &  0  & c_{3} & c_{3} & c_{2} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{1} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 &  1 \\
     1 &  0 & -1 &  0 & -1 &  0 \\
     1 &  1 &  0 &  1 & -1 & -1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 & -1 \\
    -1 &  0 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  - v_{1}  \\ v_{2} \\  - v_{1}  \\ v_{1} \\  0  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  - c_{3}  & c_{1} &  - c_{1}  &  0  &  - c_{3}  \\
    \cdot & c_{2} &  - c_{3}  & c_{3} &  0  & c_{2} \\
    \cdot & \cdot & c_{1} &  - c_{1}  &  0  &  - c_{3}  \\
    \cdot & \cdot & \cdot & c_{1} &  0  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 &  1 \\
     1 &  0 & -1 &  0 & -1 &  1 \\
     1 &  1 &  0 & -1 &  0 &  0 \\
     1 &  0 &  1 &  0 & -1 & -1 \\
    -1 &  1 &  0 &  1 &  0 &  0 \\
    -1 & -1 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  0  \\ v_{2} \\ v_{1} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  0  & c_{2} & c_{1} & c_{1} & c_{2} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{3} & c_{2} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 &  1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     1 &  0 &  0 &  0 & -1 &  0 \\
    -1 &  0 &  1 &  1 &  0 &  0 \\
    -1 &  0 &  1 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\ v_{1} \\  0  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{2} & c_{1} &  0  & c_{1} & c_{2} \\
    \cdot & c_{3} & c_{2} &  0  & c_{2} & c_{3} \\
    \cdot & \cdot & c_{1} &  0  & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 &  1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     1 &  1 &  0 &  0 & -1 &  0 \\
     1 &  0 &  0 &  0 & -1 &  0 \\
    -1 &  0 &  1 &  1 &  0 & -1 \\
    -1 &  0 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  0  \\ v_{1} \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  0  & c_{1} & c_{2} & c_{1} & c_{2} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{1} & c_{2} & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 &  1 \\
     1 &  0 & -1 &  0 &  0 &  1 \\
     1 &  1 &  0 & -1 & -1 &  0 \\
     1 &  0 &  1 &  0 &  0 & -1 \\
    -1 &  0 &  1 &  0 &  0 & -1 \\
    -1 & -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{1} \\ v_{2} \\  0  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{1} & c_{3} &  0  & c_{1} & c_{3} \\
    \cdot & \cdot & c_{2} &  0  & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 & -1 &  1 &  1 \\
     1 &  0 & -1 &  0 &  0 &  1 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     1 &  0 &  0 &  0 &  0 & -1 \\
    -1 &  0 &  1 &  0 &  0 & -1 \\
    -1 & -1 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{1} \\  2  v_{2}  \\  - v_{2}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    \frac{ 1 }{ 2 } c_{2}  & c_{3} & c_{2} & \frac{ -1 }{ 2 } c_{2}  & c_{3} & \frac{ 1 }{ 2 } c_{2}  \\
    \cdot & c_{1} &  2  c_{3}  &  - c_{3}  & c_{1} & c_{3} \\
    \cdot & \cdot &  2  c_{2}  &  - c_{2}  &  2  c_{3}  & c_{2} \\
    \cdot & \cdot & \cdot & \frac{ 1 }{ 2 } c_{2}  &  - c_{3}  & \frac{ -1 }{ 2 } c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & \frac{ 1 }{ 2 } c_{2}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 & -1 & -1 &  0 &  0 \\
     1 &  1 &  0 & -1 &  0 &  0 \\
     0 &  1 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  0  \\  0  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  0  &  0  & c_{1} & c_{2} &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 & -1 & -1 &  0 &  0 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{2} \\  0  \\  0  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} &  0  &  0  & c_{2} & c_{3} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 & -1 & -1 &  0 &  1 \\
     1 &  1 &  0 & -1 & -1 &  0 \\
     0 &  1 &  1 &  0 &  0 & -1 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
    -1 & -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  0  \\ v_{2} \\ v_{1} \\  0  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  0  & c_{3} & c_{1} &  0  & c_{3} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{2} & c_{3} &  0  & c_{2} \\
    \cdot & \cdot & \cdot & c_{1} &  0  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 & -1 & -1 &  0 &  1 \\
     1 &  1 &  0 & -1 &  0 & -1 \\
     0 &  1 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 & -1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  0  \\  0  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  0  &  0  & c_{1} & c_{2} &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 & -1 & -1 &  0 &  1 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 & -1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{2} \\  0  \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} &  0  & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 & -1 & -1 &  1 &  0 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
     0 & -1 &  1 &  0 &  0 &  1 \\
    -1 &  0 &  1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\  0  \\  2  v_{1}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    \frac{ 1 }{ 2 } c_{2}  & c_{3} &  0  & c_{2} & \frac{ 1 }{ 2 } c_{2}  & c_{3} \\
    \cdot & c_{1} &  0  &  2  c_{3}  & c_{3} & c_{1} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot &  2  c_{2}  & c_{2} &  2  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \frac{ 1 }{ 2 } c_{2}  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{1} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 & -1 & -1 &  1 &  0 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
     0 & -1 &  0 &  0 &  0 &  1 \\
    -1 &  0 &  1 &  1 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{2} \\  0  \\ v_{1} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{1} &  0  & c_{3} & c_{3} & c_{1} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{2} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{1} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 & -1 \\
     1 &  1 &  0 & -1 &  0 &  0 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{2}  \\  0  \\ v_{2} \\  2  v_{2}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     4  c_{3}  &  0  &  2  c_{3}  &  4  c_{3}  &  2  c_{2}  &  2  c_{3}  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{3} &  2  c_{3}  & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot &  4  c_{3}  &  2  c_{2}  &  2  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 & -1 \\
     1 &  1 &  0 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\  0  \\ v_{1} \\ v_{2} \\  0  \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  0  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     1 &  1 &  0 & -1 &  0 & -1 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  0  \\ v_{2} \\  0  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  0  & c_{3} &  0  & c_{2} & c_{3} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{3} &  0  & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 &  0 \\
     1 &  1 &  0 & -1 &  0 &  0 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  0  \\ v_{2} \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  0  & c_{3} & c_{3} & c_{2} & c_{3} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{3} & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 &  1 \\
     1 &  1 &  0 & -1 & -1 &  0 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
    -1 & -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\ v_{2} \\  - v_{1}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{3} &  - c_{2}  & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} &  - c_{1}  &  - c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 & -1 &  0 &  0 &  1 \\
     1 &  1 &  0 & -1 &  0 & -1 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 & -1 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\  0  \\ v_{2} \\  - v_{2}  \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{3} &  - c_{3}  & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & c_{3} &  - c_{2}  &  - c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 & -1 &  0 &  1 & -1 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 & -1 &  1 &  0 &  0 &  1 \\
    -1 &  1 &  1 &  0 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  2  v_{2}  \\  0  \\ v_{1} \\ v_{2} \\  2  v_{2}  \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  2  c_{3}  &  0  & c_{2} & c_{3} &  2  c_{3}  \\
    \cdot &  4  c_{3}  &  0  &  2  c_{2}  &  2  c_{3}  &  4  c_{3}  \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{3}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 & -1 &  0 &  1 & -1 \\
     1 &  1 &  0 &  0 & -1 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 & -1 &  1 &  0 &  0 & -1 \\
    -1 &  1 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  0  \\ v_{2} \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  0  & c_{3} & c_{2} & c_{3} & c_{3} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{3} & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 & -1 &  0 &  1 & -1 \\
     1 &  1 &  0 &  0 & -1 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 & -1 &  1 &  0 &  0 &  1 \\
    -1 &  1 &  0 &  0 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{2} \\  0  \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} &  0  & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 & -1 &  0 &  1 &  0 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 & -1 &  1 &  0 &  0 & -1 \\
    -1 &  0 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  0  \\ v_{2} \\ v_{1} \\  0  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  0  & c_{3} & c_{2} &  0  & c_{3} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{3} & c_{2} &  0  & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} &  0  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 & -1 &  0 &  1 &  0 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 & -1 &  1 &  0 &  0 &  0 \\
    -1 &  0 &  1 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{1} \\ v_{1} \\ v_{2} \\  0  \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{1} & c_{1} & c_{2} &  0  &  2  c_{1}  \\
    \cdot & c_{1} & c_{1} & c_{2} &  0  &  2  c_{1}  \\
    \cdot & \cdot & c_{1} & c_{2} &  0  &  2  c_{1}  \\
    \cdot & \cdot & \cdot & c_{3} &  0  &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 & -1 &  0 &  1 &  0 \\
     1 &  1 &  0 &  0 & -1 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 & -1 &  1 &  0 &  0 &  1 \\
    -1 &  0 &  1 &  0 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  0  \\ v_{2} \\  0  \\ v_{1} \\  0  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     0  &  0  &  0  &  0  &  0  &  0  \\
    \cdot & c_{3} &  0  & c_{2} &  0  & c_{3} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} &  0  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 &  0 & -1 & -1 &  0 \\
     1 &  0 &  0 & -1 &  0 &  0 \\
     0 &  1 &  1 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
    -1 &  0 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\  0  \\ v_{1} \\  0  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{3} &  0  & c_{1} &  0  & c_{3} \\
    \cdot & c_{2} &  0  & c_{3} &  0  & c_{2} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} &  0  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 &  0 & -1 & -1 &  0 \\
     1 &  0 &  0 & -1 &  1 &  0 \\
     0 &  1 &  1 &  0 &  0 & -1 \\
     0 &  1 & -1 &  0 &  0 & -1 \\
    -1 &  0 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\  0  \\ v_{1} \\  0  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{3} &  0  & c_{1} &  0  & c_{3} \\
    \cdot & c_{2} &  0  & c_{3} &  0  & c_{2} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} &  0  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 &  0 & -1 & -1 &  0 \\
     1 &  0 &  0 & -1 &  1 &  0 \\
     0 &  1 &  1 &  0 &  0 & -1 \\
     0 &  1 & -1 &  0 &  0 &  0 \\
    -1 &  0 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{1} \\ v_{1} \\ v_{2} \\  0  \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{2} & c_{2} & c_{1} &  0  &  2  c_{2}  \\
    \cdot & \frac{ 1 }{ 2 } c_{3}  & \frac{ 1 }{ 2 } c_{3}  & c_{2} &  0  & c_{3} \\
    \cdot & \cdot & \frac{ 1 }{ 2 } c_{3}  & c_{2} &  0  & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} &  0  &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  2  c_{3}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 &  0 & -1 & -1 &  1 \\
     1 &  0 &  0 & -1 &  0 &  0 \\
     0 &  1 &  1 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
    -1 & -1 &  0 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\  0  \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{3} &  0  & c_{1} & c_{3} & c_{3} \\
    \cdot & c_{2} &  0  & c_{3} & c_{2} & c_{2} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{1} & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{2} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 &  0 & -1 &  0 & -1 \\
     1 &  0 &  0 &  1 &  0 & -1 \\
     0 &  1 & -1 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{1}  \\ v_{1} \\ v_{1} \\  0  \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     4  c_{1}  &  2  c_{1}  &  2  c_{1}  &  0  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & c_{1} & c_{1} &  0  & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & c_{1} &  0  & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & \cdot &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 &  0 & -1 &  0 &  0 \\
     1 &  0 &  0 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\  0  \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} &  0  & c_{3} & c_{2} & c_{3} \\
    \cdot & c_{3} &  0  & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & \cdot & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -1 & -1 &  0 &  0 &  1 \\
     1 &  0 &  0 &  0 &  0 & -1 \\
     1 &  0 &  0 &  0 &  1 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 &  0 & -1 &  0 &  0 &  1 \\
    -1 &  1 &  1 &  0 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\  0  \\ v_{2} \\ v_{1} \\  0  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} &  0  & c_{3} & c_{2} &  0  & c_{3} \\
    \cdot &  0  &  0  &  0  &  0  &  0  \\
    \cdot & \cdot & c_{3} & c_{2} &  0  & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} &  0  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot &  0  &  0  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}



==> m6_ps_not45_short.tex <==
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -2 &  0 &  0 &  0 \\
     0 &  2 &  0 & -2 &  0 &  0 \\
     0 &  0 &  2 &  0 & -2 &  0 \\
     0 &  0 &  0 &  2 &  0 & -1 \\
    -1 &  0 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{1} \\ v_{2} \\ v_{1} \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{2} & \frac{ 1 }{ 2 } c_{3}  & c_{2} & \frac{ 1 }{ 2 } c_{3}  & c_{2} & c_{3} \\
    \cdot & \frac{ 1 }{ 2 } c_{1}  & \frac{ 1 }{ 2 } c_{3}  & \frac{ 1 }{ 2 } c_{1}  & \frac{ 1 }{ 2 } c_{3}  & c_{1} \\
    \cdot & \cdot & c_{2} & \frac{ 1 }{ 2 } c_{3}  & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \frac{ 1 }{ 2 } c_{1}  & \frac{ 1 }{ 2 } c_{3}  & c_{1} \\
    \cdot & \cdot & \cdot & \cdot & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  2  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -2 &  0 &  0 &  0 \\
     0 &  2 &  0 & -2 &  0 &  0 \\
     0 &  0 &  2 &  0 &  0 & -2 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  0 &  2 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{1}  \\ v_{1} \\  2  v_{1}  \\ v_{1} \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     4  c_{1}  &  2  c_{1}  &  4  c_{1}  &  2  c_{1}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & c_{1} &  2  c_{1}  & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot &  4  c_{1}  &  2  c_{1}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -2 &  0 &  0 &  0 \\
     0 &  2 &  0 & -2 &  0 &  0 \\
     0 &  0 &  2 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{1} \\ v_{1} \\ v_{1} \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{1} & c_{1} & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & c_{1} & c_{1} & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & c_{1} & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -2 &  0 &  0 &  0 \\
     0 &  2 &  0 & -1 &  0 &  0 \\
     0 &  0 &  1 &  0 & -2 &  0 \\
     0 &  0 &  0 &  2 &  0 & -2 \\
    -1 &  0 &  0 &  0 &  2 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{2}  \\ v_{1} \\  2  v_{2}  \\  2  v_{1}  \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     2  c_{2}  & \frac{ 1 }{ 2 } c_{3}  &  2  c_{2}  & c_{3} & c_{2} & c_{3} \\
    \cdot & \frac{ 1 }{ 2 } c_{1}  & \frac{ 1 }{ 2 } c_{3}  & c_{1} & \frac{ 1 }{ 4 } c_{3}  & c_{1} \\
    \cdot & \cdot &  2  c_{2}  & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot &  2  c_{1}  & \frac{ 1 }{ 2 } c_{3}  &  2  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & \frac{ 1 }{ 2 } c_{2}  & \frac{ 1 }{ 2 } c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  2  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -2 &  0 &  0 &  0 \\
     0 &  2 &  0 & -1 &  0 &  0 \\
     0 &  0 &  1 &  0 & -1 &  0 \\
     0 &  0 &  0 &  1 &  0 & -1 \\
    -1 &  0 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{1} \\ v_{2} \\  2  v_{1}  \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{2} & \frac{ 1 }{ 2 } c_{3}  & c_{2} & c_{3} & c_{2} & c_{3} \\
    \cdot & \frac{ 1 }{ 2 } c_{1}  & \frac{ 1 }{ 2 } c_{3}  & c_{1} & \frac{ 1 }{ 2 } c_{3}  & c_{1} \\
    \cdot & \cdot & c_{2} & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot &  2  c_{1}  & c_{3} &  2  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  2  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -2 &  0 &  0 &  0 \\
     0 &  2 &  0 & -1 &  0 &  0 \\
     0 &  0 &  1 &  0 &  0 & -2 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  0 &  2 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  4  v_{1}  \\ v_{1} \\  4  v_{1}  \\  2  v_{1}  \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     16  c_{1}  &  4  c_{1}  &  16  c_{1}  &  8  c_{1}  &  4  c_{2}  &  8  c_{1}  \\
    \cdot & c_{1} &  4  c_{1}  &  2  c_{1}  & c_{2} &  2  c_{1}  \\
    \cdot & \cdot &  16  c_{1}  &  8  c_{1}  &  4  c_{2}  &  8  c_{1}  \\
    \cdot & \cdot & \cdot &  4  c_{1}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -2 &  0 &  0 &  0 \\
     0 &  2 &  0 & -1 &  0 &  0 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{1}  \\ v_{1} \\  2  v_{1}  \\  2  v_{1}  \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     4  c_{1}  &  2  c_{1}  &  4  c_{1}  &  4  c_{1}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & c_{1} &  2  c_{1}  &  2  c_{1}  & c_{2} &  2  c_{1}  \\
    \cdot & \cdot &  4  c_{1}  &  4  c_{1}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & \cdot & \cdot &  4  c_{1}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -2 &  0 &  0 &  0 \\
     0 &  2 &  0 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 & -2 &  1 \\
     0 &  0 &  0 &  2 &  0 & -1 \\
    -1 &  0 &  1 & -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\ v_{1} \\ v_{2} \\ v_{2} \\  2  v_{2}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & \frac{ 1 }{ 2 } c_{2}  & c_{1} & \frac{ 1 }{ 2 } c_{2}  & \frac{ 1 }{ 2 } c_{2}  & c_{2} \\
    \cdot & \frac{ 1 }{ 2 } c_{3}  & \frac{ 1 }{ 2 } c_{2}  & \frac{ 1 }{ 2 } c_{3}  & \frac{ 1 }{ 2 } c_{3}  & c_{3} \\
    \cdot & \cdot & c_{1} & \frac{ 1 }{ 2 } c_{2}  & \frac{ 1 }{ 2 } c_{2}  & c_{2} \\
    \cdot & \cdot & \cdot & \frac{ 1 }{ 2 } c_{3}  & \frac{ 1 }{ 2 } c_{3}  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \frac{ 1 }{ 2 } c_{3}  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  2  c_{3}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -2 &  0 &  0 &  0 \\
     0 &  2 &  0 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 & -1 &  1 \\
     0 &  0 &  0 &  1 &  0 & -1 \\
    -1 &  0 &  1 & -1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{1} \\ v_{2} \\  2  v_{1}  \\  2  v_{1}  \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & \frac{ 1 }{ 2 } c_{2}  & c_{1} & c_{2} & c_{2} & c_{2} \\
    \cdot & \frac{ 1 }{ 4 } c_{3}  & \frac{ 1 }{ 2 } c_{2}  & \frac{ 1 }{ 2 } c_{3}  & \frac{ 1 }{ 2 } c_{3}  & \frac{ 1 }{ 2 } c_{3}  \\
    \cdot & \cdot & c_{1} & c_{2} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & c_{3} & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -2 &  0 &  0 &  0 \\
     0 &  2 &  0 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  1 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{1} \\ v_{2} \\ v_{3} \\ v_{4} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{5} & c_{2} & c_{5} & c_{6} & c_{7} &  2  c_{2}  \\
    \cdot & c_{1} & c_{2} & c_{3} & c_{4} &  2  c_{1}  \\
    \cdot & \cdot & c_{5} & c_{6} & c_{7} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & c_{8} & c_{9} &  2  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & c_{10} &  2  c_{4}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 &  0 & -1 \\
     0 &  1 &  0 & -1 &  0 &  0 \\
     0 &  1 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{1}  \\ v_{1} \\ v_{1} \\ v_{1} \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     4  c_{1}  &  2  c_{1}  &  2  c_{1}  &  2  c_{1}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & c_{1} & c_{1} & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & c_{1} & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 &  0 & -1 \\
     0 &  1 &  0 & -1 &  0 &  1 \\
     0 &  1 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 & -1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  3  v_{1}  \\ v_{1} \\ v_{1} \\  3  v_{1}  \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     9  c_{1}  &  3  c_{1}  &  3  c_{1}  &  9  c_{1}  &  3  c_{2}  &  6  c_{1}  \\
    \cdot & c_{1} & c_{1} &  3  c_{1}  & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & c_{1} &  3  c_{1}  & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & \cdot &  9  c_{1}  &  3  c_{2}  &  6  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 &  0 &  0 \\
     0 &  1 &  0 & -1 &  0 &  0 \\
     0 &  1 &  1 &  0 &  0 & -2 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  0 &  2 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{1}  \\ v_{1} \\  3  v_{1}  \\ v_{1} \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     4  c_{1}  &  2  c_{1}  &  6  c_{1}  &  2  c_{1}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & c_{1} &  3  c_{1}  & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot &  9  c_{1}  &  3  c_{1}  &  3  c_{2}  &  6  c_{1}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 &  0 &  0 \\
     0 &  1 &  0 & -1 &  0 &  0 \\
     0 &  1 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{1} \\ v_{1} \\ v_{1} \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{1} & c_{1} & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & c_{1} & c_{1} & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & c_{1} & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 &  0 &  0 \\
     0 &  1 &  0 & -1 &  0 &  1 \\
     0 &  1 &  1 &  0 &  0 & -2 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 & -1 &  2 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  3  v_{1}  \\ v_{1} \\  3  v_{1}  \\  3  v_{1}  \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     9  c_{1}  &  3  c_{1}  &  9  c_{1}  &  9  c_{1}  &  3  c_{2}  &  6  c_{1}  \\
    \cdot & c_{1} &  3  c_{1}  &  3  c_{1}  & c_{2} &  2  c_{1}  \\
    \cdot & \cdot &  9  c_{1}  &  9  c_{1}  &  3  c_{2}  &  6  c_{1}  \\
    \cdot & \cdot & \cdot &  9  c_{1}  &  3  c_{2}  &  6  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 &  0 &  0 \\
     0 &  1 &  0 & -1 &  0 &  1 \\
     0 &  1 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 & -1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{1}  \\ v_{1} \\ v_{1} \\  3  v_{1}  \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     4  c_{1}  &  2  c_{1}  &  2  c_{1}  &  6  c_{1}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & c_{1} & c_{1} &  3  c_{1}  & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & c_{1} &  3  c_{1}  & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & \cdot &  9  c_{1}  &  3  c_{2}  &  6  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 &  0 &  0 \\
     0 &  1 &  0 &  0 & -1 &  0 \\
     0 &  1 &  0 &  0 &  1 & -1 \\
     0 &  0 &  1 & -1 &  0 &  0 \\
    -1 &  0 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\ v_{1} \\ v_{1} \\ v_{2} \\  2  v_{2}  \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{1} & c_{3} & c_{3} & c_{1} &  2  c_{1}  \\
    \cdot & \frac{ 1 }{ 2 } c_{2}  & c_{1} & c_{1} & \frac{ 1 }{ 2 } c_{2}  & c_{2} \\
    \cdot & \cdot & c_{3} & c_{3} & c_{1} &  2  c_{1}  \\
    \cdot & \cdot & \cdot & c_{3} & c_{1} &  2  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & \frac{ 1 }{ 2 } c_{2}  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  2  c_{2}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 & -1 &  0 &  0 \\
     0 &  1 &  0 &  0 & -1 &  1 \\
     0 &  1 &  0 &  0 &  1 & -2 \\
     0 &  0 &  1 & -1 &  0 &  0 \\
    -1 &  0 & -1 &  2 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{1} \\ v_{2} \\ v_{2} \\  3  v_{1}  \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{2} & \frac{ 1 }{ 2 } c_{3}  & c_{2} & c_{2} & \frac{ 3 }{ 2 } c_{3}  & c_{3} \\
    \cdot & \frac{ 1 }{ 2 } c_{1}  & \frac{ 1 }{ 2 } c_{3}  & \frac{ 1 }{ 2 } c_{3}  & \frac{ 3 }{ 2 } c_{1}  & c_{1} \\
    \cdot & \cdot & c_{2} & c_{2} & \frac{ 3 }{ 2 } c_{3}  & c_{3} \\
    \cdot & \cdot & \cdot & c_{2} & \frac{ 3 }{ 2 } c_{3}  & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \frac{ 9 }{ 2 } c_{1}  &  3  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  2  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 & -1 \\
     0 &  1 &  0 & -2 &  0 &  0 \\
     0 &  0 &  2 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  3  v_{1}  \\  2  v_{1}  \\  2  v_{1}  \\ v_{1} \\ v_{2} \\  4  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     9  c_{1}  &  6  c_{1}  &  6  c_{1}  &  3  c_{1}  &  3  c_{2}  &  12  c_{1}  \\
    \cdot &  4  c_{1}  &  4  c_{1}  &  2  c_{1}  &  2  c_{2}  &  8  c_{1}  \\
    \cdot & \cdot &  4  c_{1}  &  2  c_{1}  &  2  c_{2}  &  8  c_{1}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  4  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  4  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  16  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 & -1 \\
     0 &  1 &  0 & -2 &  0 &  1 \\
     0 &  0 &  2 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 & -1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} \frac{ 3 }{ 2 } v_{1}  \\ v_{1} \\ v_{1} \\ \frac{ 3 }{ 2 } v_{1}  \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    \frac{ 9 }{ 4 } c_{1}  & \frac{ 3 }{ 2 } c_{1}  & \frac{ 3 }{ 2 } c_{1}  & \frac{ 9 }{ 4 } c_{1}  & \frac{ 3 }{ 2 } c_{2}  &  3  c_{1}  \\
    \cdot & c_{1} & c_{1} & \frac{ 3 }{ 2 } c_{1}  & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & c_{1} & \frac{ 3 }{ 2 } c_{1}  & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & \cdot & \frac{ 9 }{ 4 } c_{1}  & \frac{ 3 }{ 2 } c_{2}  &  3  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 & -1 \\
     0 &  1 &  0 & -1 &  0 &  0 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{1}  \\ v_{1} \\  2  v_{1}  \\ v_{1} \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     4  c_{1}  &  2  c_{1}  &  4  c_{1}  &  2  c_{1}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & c_{1} &  2  c_{1}  & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot &  4  c_{1}  &  2  c_{1}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 & -1 \\
     0 &  1 &  0 & -1 &  0 &  1 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 & -1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{1}  \\ v_{1} \\  2  v_{1}  \\  3  v_{1}  \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     4  c_{1}  &  2  c_{1}  &  4  c_{1}  &  6  c_{1}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & c_{1} &  2  c_{1}  &  3  c_{1}  & c_{2} &  2  c_{1}  \\
    \cdot & \cdot &  4  c_{1}  &  6  c_{1}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & \cdot & \cdot &  9  c_{1}  &  3  c_{2}  &  6  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 & -1 \\
     0 &  1 &  0 &  0 &  1 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 &  0 & -1 &  0 &  0 &  1 \\
    -1 &  1 &  1 &  0 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{2}  \\ v_{2} \\  2  v_{2}  \\ v_{1} \\ v_{2} \\  2  v_{2}  \end{bmatrix}
  \begin{bmatrix}
     4  c_{3}  &  2  c_{3}  &  4  c_{3}  &  2  c_{2}  &  2  c_{3}  &  4  c_{3}  \\
    \cdot & c_{3} &  2  c_{3}  & c_{2} & c_{3} &  2  c_{3}  \\
    \cdot & \cdot &  4  c_{3}  &  2  c_{2}  &  2  c_{3}  &  4  c_{3}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{3}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 &  0 \\
     0 &  1 &  0 & -2 &  0 &  0 \\
     0 &  0 &  2 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\  2  v_{1}  \\  2  v_{1}  \\ v_{1} \\ v_{2} \\  4  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} &  2  c_{1}  &  2  c_{1}  & c_{1} & c_{2} &  4  c_{1}  \\
    \cdot &  4  c_{1}  &  4  c_{1}  &  2  c_{1}  &  2  c_{2}  &  8  c_{1}  \\
    \cdot & \cdot &  4  c_{1}  &  2  c_{1}  &  2  c_{2}  &  8  c_{1}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  4  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  4  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  16  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 &  0 \\
     0 &  1 &  0 & -2 &  0 &  1 \\
     0 &  0 &  2 &  0 &  0 & -2 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 & -1 &  2 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{1} \\  2  v_{1}  \\ \frac{ 3 }{ 2 } v_{1}  \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{1} &  2  c_{1}  & \frac{ 3 }{ 2 } c_{1}  & c_{2} &  2  c_{1}  \\
    \cdot & c_{1} &  2  c_{1}  & \frac{ 3 }{ 2 } c_{1}  & c_{2} &  2  c_{1}  \\
    \cdot & \cdot &  4  c_{1}  &  3  c_{1}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & \cdot & \cdot & \frac{ 9 }{ 4 } c_{1}  & \frac{ 3 }{ 2 } c_{2}  &  3  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 &  0 \\
     0 &  1 &  0 & -1 &  0 &  0 \\
     0 &  0 &  1 &  0 & -2 &  0 \\
     0 &  0 &  0 &  2 &  0 & -1 \\
    -1 &  0 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{1} \\  2  v_{2}  \\ v_{1} \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    \frac{ 1 }{ 2 } c_{2}  & c_{3} & c_{2} & c_{3} & \frac{ 1 }{ 2 } c_{2}  &  2  c_{3}  \\
    \cdot & \frac{ 1 }{ 2 } c_{1}  &  2  c_{3}  & \frac{ 1 }{ 2 } c_{1}  & c_{3} & c_{1} \\
    \cdot & \cdot &  2  c_{2}  &  2  c_{3}  & c_{2} &  4  c_{3}  \\
    \cdot & \cdot & \cdot & \frac{ 1 }{ 2 } c_{1}  & c_{3} & c_{1} \\
    \cdot & \cdot & \cdot & \cdot & \frac{ 1 }{ 2 } c_{2}  &  2  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  2  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 &  0 \\
     0 &  1 &  0 & -1 &  0 &  0 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{1} \\  2  v_{1}  \\ v_{1} \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{1} &  2  c_{1}  & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & c_{1} &  2  c_{1}  & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot &  4  c_{1}  &  2  c_{1}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  2  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 &  0 \\
     0 &  1 &  0 & -1 &  0 &  1 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  0 & -1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{1} \\  2  v_{1}  \\  3  v_{1}  \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{1} &  2  c_{1}  &  3  c_{1}  & c_{2} &  2  c_{1}  \\
    \cdot & c_{1} &  2  c_{1}  &  3  c_{1}  & c_{2} &  2  c_{1}  \\
    \cdot & \cdot &  4  c_{1}  &  6  c_{1}  &  2  c_{2}  &  4  c_{1}  \\
    \cdot & \cdot & \cdot &  9  c_{1}  &  3  c_{2}  &  6  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 &  0 \\
     0 &  1 &  0 &  0 &  1 & -2 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 &  0 & -1 &  0 &  0 &  1 \\
    -1 &  0 &  2 &  0 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{1} \\  2  v_{1}  \\ v_{2} \\  3  v_{1}  \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{1} &  2  c_{1}  & c_{2} &  3  c_{1}  &  2  c_{1}  \\
    \cdot & c_{1} &  2  c_{1}  & c_{2} &  3  c_{1}  &  2  c_{1}  \\
    \cdot & \cdot &  4  c_{1}  &  2  c_{2}  &  6  c_{1}  &  4  c_{1}  \\
    \cdot & \cdot & \cdot & c_{3} &  3  c_{2}  &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot &  9  c_{1}  &  6  c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 &  0 \\
     0 &  1 &  0 &  0 &  1 & -1 \\
     0 &  0 &  0 &  0 & -2 &  1 \\
     0 &  0 & -1 &  2 &  0 &  0 \\
    -1 &  0 &  1 & -1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\  2  v_{1}  \\ v_{1} \\ v_{2} \\  2  v_{2}  \end{bmatrix}
  \begin{bmatrix}
    \frac{ 1 }{ 2 } c_{2}  & \frac{ 1 }{ 4 } c_{3}  & c_{2} & \frac{ 1 }{ 2 } c_{2}  & \frac{ 1 }{ 4 } c_{3}  & \frac{ 1 }{ 2 } c_{3}  \\
    \cdot & \frac{ 1 }{ 2 } c_{1}  & \frac{ 1 }{ 2 } c_{3}  & \frac{ 1 }{ 4 } c_{3}  & \frac{ 1 }{ 2 } c_{1}  & c_{1} \\
    \cdot & \cdot &  2  c_{2}  & c_{2} & \frac{ 1 }{ 2 } c_{3}  & c_{3} \\
    \cdot & \cdot & \cdot & \frac{ 1 }{ 2 } c_{2}  & \frac{ 1 }{ 4 } c_{3}  & \frac{ 1 }{ 2 } c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \frac{ 1 }{ 2 } c_{1}  & c_{1} \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  2  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 & -1 &  0 &  0 &  0 \\
     0 &  1 &  0 &  0 &  1 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 &  0 & -1 &  0 &  0 &  1 \\
    -1 &  0 &  1 &  0 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\  2  v_{2}  \\ v_{1} \\ v_{2} \\  2  v_{2}  \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} &  2  c_{3}  & c_{2} & c_{3} &  2  c_{3}  \\
    \cdot & c_{3} &  2  c_{3}  & c_{2} & c_{3} &  2  c_{3}  \\
    \cdot & \cdot &  4  c_{3}  &  2  c_{2}  &  2  c_{3}  &  4  c_{3}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & c_{3} &  2  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{3}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 &  0 &  0 &  0 & -2 \\
     0 &  0 &  0 & -2 &  1 &  0 \\
     0 &  0 &  2 &  0 & -2 &  0 \\
     0 &  0 & -1 &  2 &  0 &  0 \\
    -1 &  2 &  0 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{1}  \\ v_{1} \\  2  v_{2}  \\ v_{2} \\  2  v_{2}  \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     2  c_{1}  & c_{1} & c_{3} & \frac{ 1 }{ 2 } c_{3}  & c_{3} &  2  c_{1}  \\
    \cdot & \frac{ 1 }{ 2 } c_{1}  & \frac{ 1 }{ 2 } c_{3}  & \frac{ 1 }{ 4 } c_{3}  & \frac{ 1 }{ 2 } c_{3}  & c_{1} \\
    \cdot & \cdot & c_{2} & \frac{ 1 }{ 2 } c_{2}  & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \frac{ 1 }{ 4 } c_{2}  & \frac{ 1 }{ 2 } c_{2}  & \frac{ 1 }{ 2 } c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  2  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 &  0 &  0 &  0 & -2 \\
     0 &  0 &  0 & -2 &  1 &  0 \\
     0 &  0 &  2 &  0 & -1 &  0 \\
     0 &  0 & -1 &  1 &  0 &  0 \\
    -1 &  2 &  0 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{1}  \\ v_{1} \\ v_{2} \\ v_{2} \\  2  v_{2}  \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     2  c_{1}  & c_{1} & c_{2} & c_{2} &  2  c_{2}  &  2  c_{1}  \\
    \cdot & \frac{ 1 }{ 2 } c_{1}  & \frac{ 1 }{ 2 } c_{2}  & \frac{ 1 }{ 2 } c_{2}  & c_{2} & c_{1} \\
    \cdot & \cdot & \frac{ 1 }{ 2 } c_{3}  & \frac{ 1 }{ 2 } c_{3}  & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & \frac{ 1 }{ 2 } c_{3}  & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot &  2  c_{3}  &  2  c_{2}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  2  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 &  0 &  0 &  0 & -2 \\
     0 &  0 &  0 & -2 &  2 &  0 \\
     0 &  0 &  2 &  0 & -2 &  0 \\
     0 &  0 & -2 &  2 &  0 &  0 \\
    -1 &  2 &  0 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{1}  \\ v_{1} \\ v_{2} \\ v_{2} \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     2  c_{1}  & c_{1} & c_{2} & c_{2} & c_{2} &  2  c_{1}  \\
    \cdot & \frac{ 1 }{ 2 } c_{1}  & \frac{ 1 }{ 2 } c_{2}  & \frac{ 1 }{ 2 } c_{2}  & \frac{ 1 }{ 2 } c_{2}  & c_{1} \\
    \cdot & \cdot & c_{3} & c_{3} & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & c_{3} & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  2  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 &  0 &  0 &  0 & -2 \\
     0 &  0 &  0 & -1 &  1 &  0 \\
     0 &  0 &  1 &  0 & -1 &  0 \\
     0 &  0 & -1 &  1 &  0 &  0 \\
    -1 &  2 &  0 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{1}  \\ v_{1} \\ v_{2} \\ v_{2} \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     2  c_{1}  & c_{1} & c_{2} & c_{2} & c_{2} &  2  c_{1}  \\
    \cdot & \frac{ 1 }{ 2 } c_{1}  & \frac{ 1 }{ 2 } c_{2}  & \frac{ 1 }{ 2 } c_{2}  & \frac{ 1 }{ 2 } c_{2}  & c_{1} \\
    \cdot & \cdot & c_{3} & c_{3} & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & c_{3} & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  2  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 &  0 &  0 &  0 & -2 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  2 &  0 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{1}  \\ v_{1} \\ v_{2} \\ v_{3} \\ v_{4} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
     4  c_{1}  &  2  c_{1}  &  2  c_{2}  &  2  c_{3}  &  2  c_{4}  &  4  c_{1}  \\
    \cdot & c_{1} & c_{2} & c_{3} & c_{4} &  2  c_{1}  \\
    \cdot & \cdot & c_{5} & c_{6} & c_{7} &  2  c_{2}  \\
    \cdot & \cdot & \cdot & c_{8} & c_{9} &  2  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & c_{10} &  2  c_{4}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  4  c_{1}  \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  1 \\
     2 &  0 &  0 &  0 &  0 & -1 \\
     0 &  0 &  0 & -2 &  2 &  0 \\
     0 &  0 &  2 &  0 & -2 &  0 \\
     0 &  0 & -2 &  2 &  0 &  0 \\
    -1 &  1 &  0 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{1} \\ v_{2} \\ v_{2} \\ v_{2} \\  2  v_{1}  \end{bmatrix}
  \begin{bmatrix}
    \frac{ 1 }{ 2 } c_{1}  & \frac{ 1 }{ 2 } c_{1}  & \frac{ 1 }{ 2 } c_{3}  & \frac{ 1 }{ 2 } c_{3}  & \frac{ 1 }{ 2 } c_{3}  & c_{1} \\
    \cdot & \frac{ 1 }{ 2 } c_{1}  & \frac{ 1 }{ 2 } c_{3}  & \frac{ 1 }{ 2 } c_{3}  & \frac{ 1 }{ 2 } c_{3}  & c_{1} \\
    \cdot & \cdot & c_{2} & c_{2} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & c_{2} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot &  2  c_{1}  \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 & -2 &  0 &  0 &  0 \\
     0 &  2 &  0 & -2 &  0 &  0 \\
     0 &  0 &  2 &  0 & -2 &  0 \\
     0 &  0 &  0 &  2 &  0 & -2 \\
    -2 &  0 &  0 &  0 &  2 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\ v_{1} \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{2} & c_{3} & c_{2} & c_{3} & c_{2} & c_{3} \\
    \cdot & c_{1} & c_{3} & c_{1} & c_{3} & c_{1} \\
    \cdot & \cdot & c_{2} & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} & c_{3} & c_{1} \\
    \cdot & \cdot & \cdot & \cdot & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{1} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 & -2 &  0 &  0 &  0 \\
     0 &  2 &  0 & -2 &  0 &  0 \\
     0 &  0 &  2 &  0 &  0 & -2 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -2 &  0 &  0 &  2 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\ v_{2} \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} & c_{3} & c_{3} & c_{2} & c_{3} \\
    \cdot & c_{3} & c_{3} & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & c_{3} & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 & -2 &  0 &  0 &  0 \\
     0 &  2 &  0 & -1 &  0 & -1 \\
     0 &  0 &  1 &  0 & -1 &  0 \\
     0 &  0 &  0 &  1 &  0 & -1 \\
    -2 &  0 &  1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\ v_{1} \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{2} & c_{3} & c_{2} & c_{3} & c_{2} & c_{3} \\
    \cdot & c_{1} & c_{3} & c_{1} & c_{3} & c_{1} \\
    \cdot & \cdot & c_{2} & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} & c_{3} & c_{1} \\
    \cdot & \cdot & \cdot & \cdot & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{1} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 & -2 &  0 &  0 &  0 \\
     0 &  2 &  0 & -1 &  0 & -1 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -2 &  0 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\ v_{2} \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} & c_{3} & c_{3} & c_{2} & c_{3} \\
    \cdot & c_{3} & c_{3} & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & c_{3} & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 & -2 &  0 &  0 &  0 \\
     0 &  2 &  0 &  0 &  0 & -2 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -2 &  0 &  2 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{4} \\ v_{1} \\ v_{2} \\ v_{3} \\ v_{4} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{4} & c_{1} & c_{2} & c_{3} & c_{4} \\
    \cdot & c_{10} & c_{4} & c_{7} & c_{9} & c_{10} \\
    \cdot & \cdot & c_{1} & c_{2} & c_{3} & c_{4} \\
    \cdot & \cdot & \cdot & c_{5} & c_{6} & c_{7} \\
    \cdot & \cdot & \cdot & \cdot & c_{8} & c_{9} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{10} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 & -1 & -1 & -1 &  0 \\
     0 &  1 &  0 & -1 &  1 & -1 \\
     0 &  1 &  1 &  0 & -1 & -1 \\
     0 &  1 & -1 &  1 &  0 & -1 \\
    -2 &  0 &  1 &  1 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} \frac{ 3 }{ 2 } v_{1}  \\ v_{2} \\ v_{1} \\ v_{1} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    \frac{ 9 }{ 4 } c_{3}  & \frac{ 3 }{ 2 } c_{2}  & \frac{ 3 }{ 2 } c_{3}  & \frac{ 3 }{ 2 } c_{3}  & \frac{ 3 }{ 2 } c_{3}  & \frac{ 3 }{ 2 } c_{2}  \\
    \cdot & c_{1} & c_{2} & c_{2} & c_{2} & c_{1} \\
    \cdot & \cdot & c_{3} & c_{3} & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & c_{3} & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{1} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 & -1 & -1 &  0 &  0 \\
     0 &  1 &  0 & -1 &  1 & -1 \\
     0 &  1 &  1 &  0 & -1 & -1 \\
     0 &  0 & -1 &  1 &  0 &  0 \\
    -2 &  0 &  1 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\ v_{1} \\ v_{1} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{2} & c_{3} & c_{2} & c_{2} & c_{2} & c_{3} \\
    \cdot & c_{1} & c_{3} & c_{3} & c_{3} & c_{1} \\
    \cdot & \cdot & c_{2} & c_{2} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & c_{2} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{1} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 & -1 &  0 &  0 & -1 \\
     0 &  1 &  0 & -1 &  0 &  0 \\
     0 &  0 &  1 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -2 &  1 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\ v_{2} \\ v_{2} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} & c_{3} & c_{3} & c_{2} & c_{3} \\
    \cdot & c_{3} & c_{3} & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & c_{3} & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & c_{3} & c_{2} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & c_{1} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 &  0 &  0 &  0 & -2 \\
     0 &  0 &  0 & -2 &  2 &  0 \\
     0 &  0 &  2 &  0 & -2 &  0 \\
     0 &  0 & -2 &  2 &  0 &  0 \\
    -2 &  2 &  0 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\ v_{1} \\ v_{1} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{1} & c_{2} & c_{2} & c_{2} & c_{1} \\
    \cdot & c_{1} & c_{2} & c_{2} & c_{2} & c_{1} \\
    \cdot & \cdot & c_{3} & c_{3} & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & c_{3} & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{1} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 &  0 &  0 &  0 & -2 \\
     0 &  0 &  0 & -1 &  1 &  0 \\
     0 &  0 &  1 &  0 & -1 &  0 \\
     0 &  0 & -1 &  1 &  0 &  0 \\
    -2 &  2 &  0 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\ v_{1} \\ v_{1} \\ v_{1} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{1} & c_{2} & c_{2} & c_{2} & c_{1} \\
    \cdot & c_{1} & c_{2} & c_{2} & c_{2} & c_{1} \\
    \cdot & \cdot & c_{3} & c_{3} & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & c_{3} & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{1} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  0 &  2 \\
     2 &  0 &  0 &  0 &  0 & -2 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -2 &  2 &  0 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{4} \\ v_{4} \\ v_{1} \\ v_{2} \\ v_{3} \\ v_{4} \end{bmatrix}
  \begin{bmatrix}
    c_{10} & c_{10} & c_{4} & c_{7} & c_{9} & c_{10} \\
    \cdot & c_{10} & c_{4} & c_{7} & c_{9} & c_{10} \\
    \cdot & \cdot & c_{1} & c_{2} & c_{3} & c_{4} \\
    \cdot & \cdot & \cdot & c_{5} & c_{6} & c_{7} \\
    \cdot & \cdot & \cdot & \cdot & c_{8} & c_{9} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{10} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 &  0 &  0 \\
     0 &  1 &  0 &  0 & -2 &  1 \\
     0 &  1 &  0 &  0 &  1 & -2 \\
    -1 &  0 &  2 & -1 &  0 &  0 \\
    -1 &  0 & -1 &  2 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\ v_{1} \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{1} & c_{2} & c_{1} & c_{1} & c_{2} & c_{2} \\
    \cdot & c_{3} & c_{2} & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot & c_{1} & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 & -1 &  0 &  0 \\
     0 &  1 &  0 &  0 & -1 &  0 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
    -1 &  0 &  1 &  0 &  0 &  0 \\
    -1 &  0 &  0 &  1 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{1} \\ v_{2} \\ v_{1} \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{2} & c_{1} & c_{2} & c_{2} & c_{1} & c_{1} \\
    \cdot & c_{3} & c_{1} & c_{1} & c_{3} & c_{3} \\
    \cdot & \cdot & c_{2} & c_{2} & c_{1} & c_{1} \\
    \cdot & \cdot & \cdot & c_{2} & c_{1} & c_{1} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 &  0 & -1 & -1 \\
     0 &  1 &  0 &  0 & -1 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 & -1 \\
    -1 &  1 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{2}  \\ v_{2} \\  2  v_{2}  \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     4  c_{3}  &  2  c_{3}  &  4  c_{3}  &  2  c_{2}  &  2  c_{3}  &  2  c_{3}  \\
    \cdot & c_{3} &  2  c_{3}  & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot &  4  c_{3}  &  2  c_{2}  &  2  c_{3}  &  2  c_{3}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 &  0 & -1 & -1 \\
     0 &  1 &  0 &  0 & -1 &  1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 & -1 \\
    -1 &  1 & -1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  3  v_{2}  \\  2  v_{2}  \\  2  v_{2}  \\ v_{1} \\  3  v_{2}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     9  c_{3}  &  6  c_{3}  &  6  c_{3}  &  3  c_{2}  &  9  c_{3}  &  3  c_{3}  \\
    \cdot &  4  c_{3}  &  4  c_{3}  &  2  c_{2}  &  6  c_{3}  &  2  c_{3}  \\
    \cdot & \cdot &  4  c_{3}  &  2  c_{2}  &  6  c_{3}  &  2  c_{3}  \\
    \cdot & \cdot & \cdot & c_{1} &  3  c_{2}  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot &  9  c_{3}  &  3  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 &  0 & -1 &  0 \\
     0 &  1 &  0 &  0 & -1 &  0 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 & -1 \\
    -1 &  0 &  0 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\ v_{2} \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} & c_{3} & c_{2} & c_{3} & c_{3} \\
    \cdot & c_{3} & c_{3} & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot & c_{3} & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 &  0 & -1 &  0 \\
     0 &  1 &  0 &  0 & -1 &  1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  1 &  0 &  0 & -1 \\
    -1 &  0 & -1 &  0 &  1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{2}  \\  2  v_{2}  \\ v_{2} \\ v_{1} \\  3  v_{2}  \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     4  c_{3}  &  4  c_{3}  &  2  c_{3}  &  2  c_{2}  &  6  c_{3}  &  2  c_{3}  \\
    \cdot &  4  c_{3}  &  2  c_{3}  &  2  c_{2}  &  6  c_{3}  &  2  c_{3}  \\
    \cdot & \cdot & c_{3} & c_{2} &  3  c_{3}  & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} &  3  c_{2}  & c_{2} \\
    \cdot & \cdot & \cdot & \cdot &  9  c_{3}  &  3  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 &  0 & -1 &  0 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  0 &  0 &  0 &  0 \\
    -1 &  0 &  1 &  0 &  0 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\ v_{2} \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} & c_{3} & c_{2} & c_{3} & c_{3} \\
    \cdot & c_{3} & c_{3} & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot & c_{3} & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 &  0 & -1 &  0 \\
     0 &  1 &  0 &  0 &  0 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 &  0 &  0 &  0 &  1 \\
    -1 &  0 &  1 &  0 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{2}  \\ v_{2} \\  3  v_{2}  \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
     4  c_{3}  &  2  c_{3}  &  6  c_{3}  &  2  c_{2}  &  2  c_{3}  &  2  c_{3}  \\
    \cdot & c_{3} &  3  c_{3}  & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot &  9  c_{3}  &  3  c_{2}  &  3  c_{3}  &  3  c_{3}  \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}

\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 &  0 & -1 &  0 \\
     0 &  1 &  0 &  0 &  1 & -2 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 & -1 &  0 &  0 &  1 \\
    -1 &  0 &  2 &  0 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix} v_{2} \\ v_{2} \\ v_{2} \\ v_{1} \\ v_{2} \\ v_{2} \end{bmatrix}
  \begin{bmatrix}
    c_{3} & c_{3} & c_{3} & c_{2} & c_{3} & c_{3} \\
    \cdot & c_{3} & c_{3} & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot & c_{3} & c_{2} & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & c_{1} & c_{2} & c_{2} \\
    \cdot & \cdot & \cdot & \cdot & c_{3} & c_{3} \\
    \cdot & \cdot & \cdot & \cdot & \cdot & c_{3} \\
  \end{bmatrix}
$
}
\makebox[.01\linewidth][r]{\,}%
\parbox{.07\linewidth}{\stepcounter{mac}(\themac)}%
\resizebox{.42\linewidth}{!}{%
$
  \begin{bmatrix}
     0 & -2 &  0 &  0 &  1 &  1 \\
     2 &  0 & -1 &  0 & -1 &  0 \\
     0 &  1 &  0 &  0 &  1 & -1 \\
     0 &  0 &  0 &  0 &  0 &  0 \\
    -1 &  1 & -1 &  0 &  0 &  1 \\
    -1 &  0 &  1 &  0 & -1 &  0 \\
  \end{bmatrix}
\begin{bmatrix}  2  v_{2}  \\  2  v_{2}  \\  3  v_{2}  \\ v_{1} \\ v_{2} \\  3  v_{2}  \end{bmatrix}
  \begin{bmatrix}
     2  c_{1}  &  2  c_{1}  &  3  c_{1}  &  2  c_{3}  & c_{1} &  3  c_{1}  \\
    \cdot &  2  c_{1}  &  3  c_{1}  &  2  c_{3}  & c_{1} &  3  c_{1}  \\
    \cdot & \cdot & \frac{ 9 }{ 2 } c_{1}  &  3  c_{3}  & \frac{ 3 }{ 2 } c_{1}  & \frac{ 9 }{ 2 } c_{1}  \\
    \cdot & \cdot & \cdot & c_{2} & c_{3} &  3  c_{3}  \\
    \cdot & \cdot & \cdot & \cdot & \frac{ 1 }{ 2 } c_{1}  & \frac{ 3 }{ 2 } c_{1}  \\
    \cdot & \cdot & \cdot & \cdot & \cdot & \frac{ 9 }{ 2 } c_{1}  \\
  \end{bmatrix}
$
}


